Accordion: Adaptive Gradient Communication via Critical Learning Regime Identification

Distributed model training suffers from communication bottlenecks due to frequent model updates transmitted across compute nodes. To alleviate these bottlenecks, practitioners use gradient compression techniques like sparsification, quantization, or low-rank updates. The techniques usually require choosing a static compression ratio, often requiring users to balance the trade-off between model accuracy and per-iteration speedup. In this work, we show that such performance degradation due to choosing a high compression ratio is not fundamental. An adaptive compression strategy can reduce communication while maintaining final test accuracy. Inspired by recent findings on critical learning regimes, in which small gradient errors can have irrecoverable impact on model performance, we propose Accordion a simple yet effective adaptive compression algorithm. While Accordion maintains a high enough compression rate on average, it avoids over-compressing gradients whenever in critical learning regimes, detected by a simple gradient-norm based criterion. Our extensive experimental study over a number of machine learning tasks in distributed environments indicates that Accordion, maintains similar model accuracy to uncompressed training, yet achieves up to 5.5x better compression and up to 4.1x end-to-end speedup over static approaches. We show that Accordion also works for adjusting the batch size, another popular strategy for alleviating communication bottlenecks.

==> Tables/adasparse_param.tex <==
% \begin{wraptable}{r}{0.5\linewidth}

% \caption{Hyper-parameters for \adasp}
% \vspace{-0.1in}
% \begin{tabularx}{\linewidth}{l|X}
% \hline
% \textbf{Parameter} & \textbf{Description} \\ \hline
%     $change\_thresh$ & Threshold to determine critical regime based on rate of change of gradient norm \\ \hline
%     \textsc{switch\_freq} & Frequency to run \adasp\ to change Gradient Compression \\ \hline
%     \lc  &  Lower Compression Ratio \\ \hline
%     \hc     &  Higher Compression  Ratio \\\hline
% \end{tabularx}

% \end{wraptable}
% \vspace{-0.2in}

==> Tables/results.tex <==
\begin{table}[]
\begin{minipage}{0.485\textwidth}
\centering
\caption{ \small{\adasp\ with \powersgd\ on \cifart\ }}
\label{tab:cifar10psgd}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllllll@{}}
\toprule
\textbf{Network} &
  \textbf{Rank} &
  \textbf{Accuracy} &
  \multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Data Sent\\(Million Floats)\end{tabular}}} &
  \multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Time\\ (Seconds)\end{tabular}}} \\ \midrule
\multirow{3}{*}{Resnet-18} & Rank 2    & \textbf{94.5\%} & 2418.4 & {($1 \times$)} & {3509} & {($1 \times$)} \\ \cmidrule(l){2-7} 
                           & Rank 1    & 94.1\% & 1350.4 & ($1.7 \times$) & 3386 & {($1.03 \times$)}\\ \cmidrule(l){2-7} 
                           & \adasp & \textbf{94.5\%} & 1571.8 & {(\textbf{1.5}$\mathbf{\times}$)} & 3398 & {(\textbf{1.03}$\mathbf{\times}$)} \\ \midrule
\multirow{3}{*}{VGG-19bn}  & Rank 4    & \textbf{93.4\%} & 6752.0 & {($1 \times$)} & 3613 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                           & Rank 1    & 68.6\% & 2074.9 & {($3.25 \times$)} & 3158 & {($1.14 \times$)} \\ \cmidrule(l){2-7} 
                           & \adasp & \textbf{92.6\%} & 2945.1 & {(\textbf{2.3}$\mathbf{\times}$)} & 3220 & {(\textbf{1.12}$\mathbf{\times}$)} \\ \midrule
\multirow{3}{*}{Senet}     & Rank 4    & \textbf{94.5\%}& 4361.3 & {($1 \times$)} & 4689 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                           & Rank 1    & 94.2\% & 1392.6 & {($3.1 \times$)} & 4134 & {($1.13 \times$)} \\ \cmidrule(l){2-7} 
                           & \adasp & \textbf{94.5\%} & 2264.4 & {(\textbf{1.9}$\mathbf{\times}$)} & 4298 & {(\textbf{1.09}$\mathbf{\times}$)} \\ \bottomrule
\end{tabular}}
\end{minipage}\quad
\begin{minipage}{0.49\textwidth}
\centering
\caption{\small{\adasp\ with\hspace{0.01cm}\powersgd\ on \cifarh }}
\label{tab:cifar100psgd}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllllll@{}}
\toprule
\textbf{Network} &
  \textbf{Rank} &
  \textbf{Accuracy} &
  \multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Data Sent\\(Million Floats)\end{tabular}}} &
  \multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Time\\ (Seconds)\end{tabular}}} \\ \midrule
\multirow{3}{*}{Resnet-18} & Rank 2    & \textbf{71.7}\% & 2426.3 & {($1 \times$)} & 3521 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                           & Rank 1    & 70.0\% & 1355.7 & {($1.8 \times$)} & 3388 & {($1.04 \times$)}\\ \cmidrule(l){2-7} 
                           & \adasp & \textbf{71.8}\% & 1566.3 & {(\textbf{1.6}$\mathbf{\times}$)} & 3419 & {(\textbf{1.03}$\mathbf{\times}$)} \\ \midrule
\multirow{3}{*}{DenseNet}  & Rank 2    & \textbf{72.0\%} & 3387.4 & {($1 \times$)} & 13613 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                           & Rank 1    & 71.6\% & 2155.6 & {($1.6 \times$)} & 12977 & {($1.04 \times$)} \\ \cmidrule(l){2-7} 
                           & \adasp & \textbf{72.5\%} & 2284.9 & {(\textbf{1.5}$\mathbf{\times}$)} & 13173 & {(\textbf{1.03}$\mathbf{\times}$)} \\ \midrule
\multirow{3}{*}{Senet}     & Rank 2    & \textbf{72.5\%} & 2878.1 & {($1 \times$)} & 5217 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                           & Rank 1    & 71.5\% & 1683.1 & {($1.7 \times$)} & 4994 & {($1.04 \times$)} \\ \cmidrule(l){2-7} 
                           & \adasp & \textbf{72.4\%} & 2175.6 & {(\textbf{1.3}$\mathbf{\times}$)} & 5074 & {(\textbf{1.03}$\times$)} \\ \bottomrule
% \multirow{3}{*}{Wideresnet} & Rank 2   & 75.7\% & 2878.1 & {\color{gray}($1 \times$)} & 4978 & {\color{gray}($1 \times$)} \\ \cmidrule(l){2-7} 
%                           & Rank 1    & 74.6\% & 1683.1 & {\color{gray}($1 \times$)} & 5180 & {\color{gray}($1 \times$)} \\ \cmidrule(l){2-7} 
%                           & Adasparse & 75.3\% & 2175.6 & {\color{gray}($1 \times$)} & 5051 & {\color{gray}($1 \times$)} \\ \bottomrule
                           
\end{tabular}}
\end{minipage}
\vspace{-0.2in}
\end{table}


\begin{table}[]
\begin{minipage}{0.485\textwidth}
\caption{\small{\adasp\ using \topk\ on \cifart\ } }
\label{tab:cifar10topk}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lllllll@{}}
\toprule
\textbf{Network} &
  \textbf{K(\%)} &
  \textbf{Accuracy} &
  \multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Data Sent\\(Billion Floats)\end{tabular}}} &
  \multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Time\\ (Seconds)\end{tabular}}} \\ \midrule
\multirow{3}{*}{Resnet-18} & 99    & \textbf{94.2\%} & 2626.1 & {($1 \times$)} & 33672 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                          & 10    & 93.1\% & 262.8 & {($9.9 \times$)} & 7957 & {($4.2 \times$)}\\ \cmidrule(l){2-7} 
                          & \adasp & \textbf{93.9\%} & 976.7 & {(\textbf{2.8}$\mathbf{\times}$)} & 9356 & {(\textbf{3.6}$\mathbf{\times}$)} \\ \midrule
\multirow{3}{*}{GoogleNet}  & 99   & \textbf{94.6\%} & 1430.9 & {($1 \times$)} & 28476 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                          & 10    & 94.1\% & 145.2 & {($9.8 \times$)} & 13111 & {($2.1 \times$)} \\ \cmidrule(l){2-7}
                          & \adasp & \textbf{94.7\%} & 383.8 & {(\textbf{3.7}$\mathbf{\times}$)} & 16022 & {(\textbf{1.7}$\mathbf{\times}$)} \\ \midrule
\multirow{3}{*}{Senet}     & 99    & \textbf{94.6\%} & 2648.7 & {($1 \times$)} & 29977 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                          & 10    & 93.8\% & 267.9 & {($9.8 \times$)} & 8055 & {($3.7 \times$)} \\ \cmidrule(l){2-7} 
                          & \adasp & \textbf{94.5\%} & 869.8 & {(\textbf{3.0}$\mathbf{\times}$)} & 13071 & {(\textbf{2.29}$\mathbf{\times}$)} \\ \bottomrule

\end{tabular}}                           
\end{minipage}\quad
\vspace{-0.1in}
\begin{minipage}{0.49\textwidth}
%\end{table}
%\begin{table}[]
\caption{\small{\adasp\ using \topk\ on \cifarh\ }}
\label{tab:cifar100topk}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lllllll@{}}
\toprule
\textbf{Network} &
  \textbf{K(\%)} &
  \textbf{Accuracy} &
  \multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Data Sent\\(Billion Floats)\end{tabular}}} &
  \multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Time\\ (Seconds)\end{tabular}}} \\ \midrule
\multirow{3}{*}{Resnet-18} & 99    & \textbf{72.4\%} & 2636.9 & {($1 \times$)} & 53460 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                          & 25    & 71.3\% & 659.4 & {($3.9 \times$)} & 6176 & {($8.6 \times$)}\\ \cmidrule(l){2-7} 
                          & \adasp & \textbf{72.3\%} & 923.6 & {(\textbf{2.8}$\mathbf{\times}$)} & 14223 & {(\textbf{3.8}$\mathbf{\times}$)} \\ \midrule
\multirow{3}{*}{GoogleNet}  & 99   & \textbf{76.2\%} & 1452.4 & {($1 \times$)} & 28579 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                          & 25    & 75.3\% & 367.3 & {($3.9 \times$)} & 12810 & {($2.23 \times$)} \\ \cmidrule(l){2-7}
                          & \adasp & \textbf{76.2\%} & 539.9 & {(\textbf{2.7}$\mathbf{\times}$)} & 15639 & {(\textbf{1.82}$\mathbf{\times}$)} \\ \midrule
\multirow{3}{*}{Senet}     & 99    & \textbf{72.8\%} & 2659.5 & {($1 \times$)} & 30312 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                          & 25    & 71.9\% & 671.9 & {($3.9 \times$)} & 7376 & {($4.1 \times$)} \\ \cmidrule(l){2-7} 
                          & \adasp & \textbf{72.7\%} & 966.13 & {(\textbf{2.8}$\mathbf{\times}$)} & 10689 & {(\textbf{2.8}$\mathbf{\times}$)} \\ \bottomrule
                           
\end{tabular}}
\end{minipage}
\end{table}

\begin{table}[]
\begin{minipage}{0.485\textwidth}
\caption{\small{\adasp\ switching Batch Size on \cifart\ } }
\label{tab:cifar10batch}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lllllll@{}}
\toprule
\textbf{Network} &
  \textbf{K(\%)} &
  \textbf{Accuracy} &
  \multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Data Sent\\(Billion Floats)\end{tabular}}} &
  \multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Time\\ (Seconds)\end{tabular}}} \\ \midrule
\multirow{3}{*}{Resnet-18} & 512    & \textbf{94.5\%} & 326.5 & {($1 \times$)} & 5009 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                          & 4096    & 93.2\% & 40.22 & {($8 \times$)} & 1721 & {($2.9 \times$)}\\ \cmidrule(l){2-7} 
                          & \adasp & \textbf{94.4\%} & 59.22 & {(\textbf{5.6}$\mathbf{\times}$)} & 1959 & {(\textbf{2.5}$\mathbf{\times}$)} \\ \midrule
\multirow{3}{*}{GoogLeNet}  & 512   & \textbf{94.7\%} & 181.28 & {($1 \times$)} & 12449 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                          & 4096    & 93.1\% & 22.19 & {($8.1 \times$)} & 3386 & {($3.67 \times$)} \\ \cmidrule(l){2-7}
                          & \adasp & \textbf{94.7\%} & 32.68 & {(\textbf{5.5}$\mathbf{\times}$)} & 6220 & {(\textbf{2.0}$\mathbf{\times}$)} \\ \midrule
\multirow{3}{*}{DenseNet}     & 512    & \textbf{93.9\%} & 29.4 & {($1 \times$)} & 14489 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                          & 4096    & 93.1\% & 3.6 & {($8.1 \times$)} & 2759 & {($5.2 \times$)} \\ \cmidrule(l){2-7} 
                          & \adasp & \textbf{94.0\%} & 5.3 & {(\textbf{5.5}$\mathbf{\times}$)} & 3547 & {(\textbf{4}$\mathbf{\times}$)} \\ \bottomrule

\end{tabular}}                           
\end{minipage}\quad
\vspace{-0.1in}
\begin{minipage}{0.49\textwidth}
%\end{table}
%\begin{table}[]
\caption{\small{\adasp\ switching Batch Size on \cifarh\ }}
\label{tab:cifar100batch}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lllllll@{}}
\toprule
\textbf{Network} &
  \textbf{K(\%)} &
  \textbf{Accuracy} &
  \multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Data Sent\\(Billion Floats)\end{tabular}}} &
  \multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Time\\ (Seconds)\end{tabular}}} \\ \midrule
\multirow{3}{*}{Resnet-18} & 512    & \textbf{74.1\%} & 326.5 & {($1 \times$)} & 5096 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                          & 4096    & 70.0\% & 40.39 & {($8 \times$)} & 1635 & {($3.1 \times$)}\\ \cmidrule(l){2-7} 
                          & \adasp & \textbf{74.3\%} & 54.96 & {(\textbf{5.5}$\mathbf{\times}$)} & 1852 & {(\textbf{2.7}$\mathbf{\times}$)} \\ \midrule
\multirow{3}{*}{GoogleNet}  & 512   & \textbf{78.0\%} & 182.1 & {($1 \times$)} & 12443 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                          & 4096    & 73.7\% & 22.5 & {($8.1\times$)} & 5755 & {($2.1 \times$)} \\ \cmidrule(l){2-7}
                          & \adasp & \textbf{78.0\%} & 33.1 & {(\textbf{5.4}$\mathbf{\times}$)} & 6228 & {(\textbf{2.0}$\mathbf{\times}$)} \\ \midrule
\multirow{3}{*}{DenseNet}     & 512    & \textbf{73.7\%} & 30.126 & {($1 \times$)} & 14928 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                          & 4096    & 70.0\% & 3.72 & {($8 \times$)} & 2775 & {($5.3 \times$)} \\ \cmidrule(l){2-7} 
                          & \adasp & \textbf{73.9\%} & 5.48 & {(\textbf{5.4}$\mathbf{\times}$)} & 3585 & {(\textbf{4.1}$\mathbf{\times}$)} \\ \bottomrule
                           
\end{tabular}}
\end{minipage}
\end{table}



==> Tables/results_2.tex <==
\begin{table}[]
\begin{minipage}{0.485\textwidth}
\caption{\small{\adasp\ using \topk\ on \cifart\ } }
\label{tab:cifar10topk}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lllllll@{}}
\toprule
\textbf{Network} &
  \textbf{K(\%)} &
  \textbf{Accuracy} &
  \multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Data\\ Sent(B)\end{tabular}}} &
  \multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Time\\ (Seconds)\end{tabular}}} \\ \midrule
\multirow{3}{*}{Resnet-18} & 99    & \textbf{94.2\%} & 2626.1 & {($1 \times$)} & 33672 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                          & 10    & 93.1\% & 262.8 & {($9.9 \times$)} & 7957 & {($4.2 \times$)}\\ \cmidrule(l){2-7} 
                          & Adasparse & \textbf{93.9\%} & 976.7 & {(\textbf{2.8}$\mathbf{\times}$)} & 9356 & {(\textbf{3.6}$\mathbf{\times}$)} \\ \midrule
\multirow{3}{*}{GoogleNet}  & 99   & \textbf{94.6\%} & 1430.9 & {($1 \times$)} & 28476 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                          & 10    & 94.1\% & 145.2 & {($9.8 \times$)} & 13111 & {($2.1 \times$)} \\ \cmidrule(l){2-7}
                          & Adasparse & \textbf{94.7\%} & 383.8 & {(\textbf{3.7}$\mathbf{\times}$)} & 16022 & {(\textbf{1.7}$\mathbf{\times}$)} \\ \midrule
\multirow{3}{*}{Senet}     & 99    & \textbf{94.6\%} & 2648.7 & {($1 \times$)} & 29977 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                          & 10    & 93.8\% & 267.9 & {($9.8 \times$)} & 8055 & {($3.7 \times$)} \\ \cmidrule(l){2-7} 
                          & Adasparse & \textbf{94.5\%} & 869.8 & {(\textbf{3.0}$\mathbf{\times}$)} & 13071 & {(\textbf{2.29}$\mathbf{\times}$)} \\ \bottomrule

\end{tabular}}                           
\end{minipage}\quad
\vspace{-0.1in}
\begin{minipage}{0.49\textwidth}
%\end{table}
%\begin{table}[]
\caption{\small{\adasp\ using \topk\ on \cifarh\ }}
\label{tab:cifar100topk}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lllllll@{}}
\toprule
\textbf{Network} &
  \textbf{K(\%)} &
  \textbf{Accuracy} &
  \multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Data\\ Sent(B)\end{tabular}}} &
  \multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Time\\ (Seconds)\end{tabular}}} \\ \midrule
\multirow{3}{*}{Resnet-18} & 99    & \textbf{72.4\%} & 2636.9 & {($1 \times$)} & 53460 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                          & 25    & 71.3\% & 659.4 & {($3.9 \times$)} & 6176 & {($8.6 \times$)}\\ \cmidrule(l){2-7} 
                          & Adasparse & \textbf{72.3\%} & 923.6 & {(\textbf{2.8}$\mathbf{\times}$)} & 14223 & {(\textbf{3.8}$\mathbf{\times}$)} \\ \midrule
\multirow{3}{*}{GoogleNet}  & 99   & \textbf{76.2\%} & 1452.4 & {($1 \times$)} & 28579 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                          & 25    & 75.3\% & 367.3 & {($3.9 \times$)} & 12810 & {($2.23 \times$)} \\ \cmidrule(l){2-7}
                          & Adasparse & \textbf{76.2\%} & 539.9 & {(\textbf{2.7}$\mathbf{\times}$)} & 15639 & {(\textbf{1.82}$\mathbf{\times}$)} \\ \midrule
\multirow{3}{*}{Senet}     & 99    & \textbf{72.8\%} & 2659.5 & {($1 \times$)} & 30312 & {($1 \times$)} \\ \cmidrule(l){2-7} 
                          & 25    & 71.9\% & 671.9 & {($3.9 \times$)} & 7376 & {($4.1 \times$)} \\ \cmidrule(l){2-7} 
                          & Adasparse & \textbf{72.7\%} & 966.13 & {(\textbf{2.8}$\mathbf{\times}$)} & 10689 & {(\textbf{2.8}$\mathbf{\times}$)} \\ \bottomrule
                           
\end{tabular}}
\end{minipage}
\end{table}

==> adasparse.tex <==
\section{AdaSparse}

\begin{figure*}[t]
    \begin{center}
    \begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{Figures/critical_regions_resnet18_cifar100.pdf}
    \caption{Critical Regimes}
     \label{fig:crit_res18_cifar100}
    \end{subfigure}
    \begin{subfigure}[b]{0.66\textwidth}
    \includegraphics[width=\textwidth]{Figures/accuracy_critical_regions_resnet18_cifar100_full_rank.pdf}
    \caption{Accuracy vs Epochs and Floats Communicated}
    \label{fig:critical_regimes_full_rank}
    \end{subfigure}
    \end{center}
    \caption{\small{\textbf{Effect of gradient compression in Critical Regimes when Training ResNet-18 on \cifarh:} (a) Critical regimes in \cifarh, ResNet-18 (b, Left) Accuracy vs Epochs. Show the significance of critical regimes in training, using low compression(Rank 2) in critical regimes is enough to get similar accuracy as using low compression throughout . (b, Right) Accuracy vs Floats Communicated, Even when we use uncompressed (Full Rank)  gradients everywhere but use high compression (Rank 1) in critical regimes  it is not possible to bridge accuracy gap.}}
    \vspace{-0.22in}
\end{figure*}

In this section, we first explain why adaptive gradient communication can help maintain a high generalization performance while minimizing the communication cost. \shivaram{I think this flow needs to change. the last section ends with goal of designing an algorithm - but that comes last. I think we can move the connection lemma stuff further behind?}
% schedule keeping
In a limited setting, we also reveal interesting connections between compression ratio and batch size, and show how the presence of critical regimes affects the choices of these parameters.
Based on these findings, we design our adaptive compression scheduling algorithm called \adasp.

% Effective adaptive compression schedule and the c
\subsection{Connection of adaptive compression to critical regimes}
\label{sec:critical_connection}
% We first show the existence of an efficient adaptive compression rate schedule.
% To design a effective compression rate schedule, we first observe how the gradient behaves while training.
% Shown in Figure~\ref{fig:critical_grad} are the experimental results with ResNet-18 on CIFAR10.
% We note that the gradient norm rapidly decreases in the first $20$ epochs and in the $10$ epochs right after the $150$-th epoch, i.e., the point at which learning rate decay occurs. 
% This implies that those regimes are the important regimes where the SGD algorithm navigates the steeper parts of the loss surface.
% Thus, if highly compressed gradients are used in these regimes, then the training algorithm might take a different trajectory than what SGD would have taken originally, and eventually get stuck in a sub-optimal minima leading to degradation in final test accuracy. 
% Based on this observation, we tried the following time-varying compression rate schedule: $\ell = \textsc{low compression rate}$ for the first $20$ epochs and for $10$ epochs after the $150$ epoch, and $\ell = \textsc{high compression rate}$ elsewhere.
% Under this schedule, gradients will not be highly distorted in the important regimes, but at the same time, the overall communication cost is almost as low as that of a strategy where a low compression rate is fixed throughout training. 
% Shown in Figure~\ref{fig:1a} are our experimental results with ResNet-18 on CIFAR10. 
% One can see that this carefully chosen compression rate schedule does not hurt the final test accuracy while significantly speeding up the training procedure due to its low communication overhead.
% ~\cite{achille2018critical, jastrzebski2018on}
%We first show the existence of an efficient adaptive compression rate schedule.
To design an effective compression rate schedule, we first observe how the gradient norm for each layer behaves while training.
When training ResNet-18 on \cifarh, in Figure~\ref{fig:crit_res18_cifar100} we see two regions where gradient norm decreases rapidly; during the first $20$ epochs and the $10$ epochs right after the $150$-th epoch, \ie{}, the point at which learning rate decay occurs. We experimentally verify that these two regions are critical by considering the following compression schedule $\ell = \textsc{low}$ for the first $20$ epochs and for $10$ epochs after the $150$ epoch, and $\ell = \textsc{high}$ elsewhere. Under this scheme the gradients will not be over-compressed in the critical regimes, but at the same time the overall communication will be close to high compression. Figure~\ref{fig:critical_regimes_full_rank} shows the experimental results with ResNet-18 on \cifarh\ for the above scheme. It can be observed that just using low compression (rank 2) in these critical regimes and high compression (rank 1) elsewhere is sufficient to get the same accuracy as using low compression throughout while reducing communication significantly.
% using a number of different schemes test
%and the communication budget has reduced significantly.
% throughout are 

Interestingly we also observe in Figure~\ref{fig:critical_regimes_full_rank} that any loss in accuracy by using high compression in critical regimes is not recoverable by using low compression elsewhere. For instance, consider the following compression schedule: $\ell = \textsc{high compression rate}$ for first $20$ epochs and for $10$ epochs after the $150$ epoch, and $\ell = \textsc{no compression}$ elsewhere.
% To further strengthen our hypothesis, 
Under this schedule, gradients will be over-compressed in the critical regimes, but will be \emph{uncompressed} elsewhere. We see that for ResNet-18 on \cifarh\ even with significantly higher communication one can not overcome the damage done to training by over compressing in critical regimes.
We hypothesize that in critical regimes, SGD is navigating to the steeper parts of the loss surface and if we use over-compressed gradients in these regimes, then the training algorithm might take a different trajectory than what SGD would have taken originally. This might cause training to reach a sub-optimal minima leading to degradation in final test accuracy. 

%that our hypothesis holds, showing that 

%\shivaram{It might also be interesting to claim here that we also see that using a simple indicator like gradient norm proves to be sufficient. Thus we both prove existence and a simple to compute indicator.}
% how in Figure~\ref{fig:critical_regimes_full_rank} 

% \begin{figure*}[t]
%     \begin{center}
%     \begin{subfigure}[b]{0.33\textwidth}
%     \includegraphics[width=\textwidth]{Figures/critical_regions_resnet18_cifar100.pdf}
%     \caption{Critical Regimes}
%      \label{fig:crit_res18_cifar100}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.66\textwidth}
%     \includegraphics[width=\textwidth]{Figures/accuracy_critical_regions_resnet18_cifar100_full_rank.pdf}
%     \caption{Accuracy vs Epochs and Floats Communicated}
%     \label{fig:critical_regimes_full_rank}
%     \end{subfigure}
%     \end{center}
%     \caption{\small{\textbf{Effect of gradient compression in Critical Regimes when Training ResNet-18 on \cifarh:} (a) Critical regimes in \cifarh, ResNet-18 (b, Left) Accuracy vs Epochs. Show the significance of critical regimes in training, using low compression(Rank 2) in critical regimes is enough to get similar accuracy as using low compression throughout . (b, Right) Accuracy vs Floats Communicated, Even when we use uncompressed (Full Rank)  gradients everywhere but use high compression (Rank 1) in critical regimes  it is not possible to bridge accuracy gap.}}
%     \vspace{-0.22in}
% \end{figure*}

\begin{figure*}[t]
    \begin{center}
    
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{Figures/critical_regime_hessian.pdf}
        \caption{Critical Regimes based on Hessian}
        \vspace{-0.1in}
        \label{fig:critical_hessian}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{Figures/critical_regions_resnet18.pdf}
        \caption{Critical Regimes based of Gradient Norm}
        \vspace{-0.1in}
        \label{fig:critical_grad}
    \end{subfigure}
    \end{center}
    \caption{\small{\textbf{Comparison of Critical Regimes found using Analysis of eigenvalues of Hessian vs Using the Norm of the Gradient:}} The experiment is performed on ResNet-18, for \cifart. We show that Critical Regimes detected by rapid decay in top eigenvalues of Hessian can also be detected using decay in gradient norm}
    \label{fig:critical_compare}
    \vspace{-0.2in}
\end{figure*}
% \begin{figure}[t]
%     \begin{center}
%     \begin{subfigure}[b]{0.33\textwidth}
%         \includegraphics[width=\textwidth]{Figures/topk_overlap.pdf}
%         \caption{Overlap in coordinates }
%         \vspace{-0.1in}
%         \label{fig:topk_overlap}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.66\textwidth}
%         \includegraphics[width=\textwidth]{Figures/critical_regions_resnet18_cifar10_batch_size_4096.pdf}
%         \caption{Critical Regions}
%         \vspace{-0.1in}
%         \label{fig:critical_batchsize}
%     \end{subfigure}
%     \end{center}
%     \caption{\small{\textbf{Effect of Batch size in Critical Regimes when Training ResNet-18 on \cifart:} (a) We show that there is significant overlap among the \textsc{Top}10\% coordinates (b, left) Shows that using small batches only in critical regimes is enough to get performance similar to using small batches everywhere. We scale learning rate linearly with batch size as suggested by~\cite{goyal2017accurate}, at steps 150 and 250 we decay the learning rate by 10 and 100 respectively \ie LR for Batch size 512 becomes 0.04 at 150th epoch. (b, right) Accuracy vs Floats Communicated}}
    
%     \label{fig:critical_regimes}
%     \vspace{-0.1in}
% \end{figure}

\noindent\textbf{Connection to critical regimes}
We next discuss how our adaptive compression strategy is closely related to the findings made in~\cite{achille2018critical, jastrzebski2018on} about critical regimes in training.
\citet{achille2018critical} showed the importance of the early phase of training, which they termed as a \emph{critical regime}. In particular, they trained a DNN with corrupted training data just for the first few epochs, and then continued training the DNN with clean training data for the rest of the epochs.
Surprisingly, the DNN trained this way showed a significantly impaired generalization performance no matter how long it was trained with the clean data after the critical regime. 
Our finding is related to this phenomenon, and further we show that not just the early phase of the training, but also the early phase after each learning rate decay is critical. \citet{jastrzebski2018on} used change in eigenvalues of the Hessian as an indicator of critical regimes, while our work proposes using change in gradient norm as an indicator.
In Figure~\ref{fig:critical_compare}, we show that these two approaches yield similar results for ResNet-18 on \cifart, with the latter having an advantage of being orders of magnitude faster to compute.

Thus, we empirically show that finding an effective communication schedule is akin to finding critical regimes in neural network training and these \textit{critical regimes} can be identified by measuring the gradient norm. 

% crudely rapid decrease in 
% if we over-compress gradients during critical regimes (epoch $1$ to epoch $10$ and epoch $150$ to epoch $170$), then the final test accuracy is significantly impaired.
% On the other hand, we show that when compression ratios are selected conservatively to avoid impairing the training process during these critical regimes, then test error is unaffected, even if high compression is used in other regimes.

\subsection{Connection to adaptive batch-size scheduling}
\label{sec:batchsize_connection}
%We compare the critical regimes identified in prior work~\cite{jastrzebski2018on} with the regions identified by rapid changes in gradient norm in Figure~\ref{fig:critical_compare}. We observe that decay in gradient norm follows a similar pattern as  which was used by \citet{jastrzebski2018on} use decay in Eigenvalues of the Hessian as an indicator of critical regimes
 
\begin{figure*}[t]
    \begin{center}
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{Figures/topk_overlap.pdf}
        \caption{Overlap in coordinates }
        \vspace{-0.1in}
        \label{fig:topk_overlap}
    \end{subfigure}
    \begin{subfigure}[b]{0.66\textwidth}
        \includegraphics[width=\textwidth]{Figures/critical_regions_resnet18_cifar10_batch_size_4096.pdf}
        \caption{Effect of Different Batch sizes in critical regimes}
        \vspace{-0.1in}
        \label{fig:critical_batchsize}
    \end{subfigure}
    % \begin{subfigure}[b]{0.9\textwidth}
    %     \includegraphics[width=0.9\textwidth]{Figures/psgd_senet_cifar10.pdf}
    %     \caption{Cifar10, SeNet}
    % \end{subfigure}
    \end{center}
    \caption{\small{\textbf{Effect of batch size (ResNet-18 on \cifart):} (a) We show that there is significant overlap among the \textsc{Top}10\% coordinates. (b, left) Shows that using small batches only in critical regimes is enough to get performance similar to using small batches everywhere. We scale learning rate linearly with batch size as in~\cite{goyal2017accurate}, at steps 150 and 250 we decay the learning rate by 10 and 100 respectively. (b, right) accuracy vs communication.}}
    
    \label{fig:critical_regimes}
    \vspace{-0.1in}
\end{figure*}

%Our experimental results also show that such critical regimes are easy-to-detect by inspecting the change in gradient norms.  See Section~\ref{} for more experimental results. \shivaram{it might be good to include these results inline here instead of in eval?} \kw{True :)}

% \subsection{Connection to batch-size scheduling~\cite{}}
We also find that there exists an implicit connection between our findings and adaptive batch-size tuning~\cite{smith2017don, devarakonda2017adabatch}.
It is well known that SGD with large batch size hurts generalization~\cite{smith2017don, yin2017gradient,keskar2016large, yao2018hess, goyal2017accurate, golmant2018computational, shallue2018measuring}. 
However, recent work~\cite{devarakonda2017adabatch} shows that one may gradually increase the batch size while training without hurting the generalization performance.
We interpret these results through the lens of \emph{critical regimes}: using small batch sizes in critical regimes, but increasing batch sizes elsewhere does not hurt the generalization performance. We empirically show this is indeed true in Figure~\ref{fig:critical_batchsize}.
%But the choice of batch sizes in non-critical regimes do not affect the generalization performance much. 

% One should use
The connection between compression and batch size tuning can be made more formal under the following assumption: ``each stochastic gradient is the sum of a sparse mean and a dense noise'', i.e.,\
\begin{equation}
\begin{split}
\nabla_w \ell(w;x_i,y_i)& = \underbrace{\mathbb{E}_j \nabla_w \ell(w;x_j,y_j)}_{\text{sparse, large magnitudes}}\\  &+\underbrace{(\nabla_w \ell(w;x_i,y_i)-\mathbb{E}_j \nabla_w \ell(w;x_j,y_j))}_{\text{dense, small magnitudes}}
\end{split}
\end{equation}

Under this assumption, we can see that ``large batch gradient $\approx$ highly compressed gradient'', as a large batch gradient will be close to $\mathbb{E}_j \nabla_w \ell(w;x_j,y_j)$ by the law of large numbers, and a highly compressed gradient will also pick up the same sparse components. 
Similarly, a small batch gradient is equivalent to weakly compressed gradient. 

To see when this assumption on gradients becomes valid, consider the following LASSO example whose goal is to minimize $\sfrac{1}{2}\cdot\|Xw - y\|_2^2 + \lambda \|w\|$, where positive-class data points $x_{+} \sim \mathcal{N}(\mu, \sigma^2 I)$, negative-class data points $x_{-} \sim \mathcal{N}(-\mu, \sigma^2 I)$, and $P(Y=+1)=P(Y=-1)=\sfrac{1}{2}$.
Here, $w$ is sparse for a properly chosen value of $\lambda$ due to the shrinkage operation~\cite{lasso}.
Then, we have the following lemma, which implies that the gradient modeling described above holds w.h.p.
\begin{lemma}\label{lem:1}
If $\mu$ is $k_1$-sparse and $w$ is $k_2$-sparse, $\mathbb{E}_j \nabla_w \ell(w;x_j,y_j)$ is $k_1 + k_2$-sparse. Let us denote by $\gamma$ the minimum absolute value of non-zero entries of $\mathbb{E}_j \nabla_w$.
Then, for any positive integer $n$ and $\epsilon > 0$, there exists a sufficiently small enough $\sigma > 0$ such that $\mathbb{P}(\max_{i \in [n]}\|\nabla_w \ell(w;x_i,y_i)-\mathbb{E}_j \nabla_w \ell(w;x_j,y_j)\|_{\infty} < \gamma) = 1-\epsilon$.
\end{lemma}

The proof can be found in the Appendix. 
We will like to point that this assumption doesn't hold for all models and data, but only does so when training is performed with sparsity inducing norms. However we conduct a simple experiment to support our intuition by collecting all stochastic gradients in an epoch and compute the overlap in coordinates of top-$10\%$ entries to find how much their supports overlap.
Figure~\ref{fig:topk_overlap} shows that $>90\%$ of the top-$K$ entries are common between a pair of stochastic gradients, thereby justifying the above gradient modeling. 

Thus, our findings along with prior work in literature can be summarized as high gradient compression, noisy training data, \emph{or} large batch size in the critical regimes of training hurts generalization. 
Although the proof is under a very limited setting and we don't claim it will hold for all models or data, our experimental results in ~\Cref{fig:topk_overlap} indicate that this might be more widely applicable. Further in Section~\ref{sec:eval} we show that \adasp\  is also able to switch between large and small Batch Size without loosing any accuracy or requiring any hyper-parameter tuning.
% already-known  performance

% in critical regimes
% \ie LR for Batch size 512 becomes 0.04 at 150th epoch
% In this section, we describe why adaptive gradient compression 
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.8\textwidth]{Figures/critical_regions_resnet18_cifar10_batch_size_4096.pdf}
%     \caption{\small{\textbf{Effect of Batch Size in Critical Regimes when Training ResNet-18 on \cifart:} (left) Accuracy vs Epochs , (Right) Accuracy vs Communication  }}
%     \label{fig:batch_4096_critical}
% \end{figure}



\subsection{\adasp}
We now provide a description of \adasp, our proposed algorithm that automatically switches between lower and higher communication levels by detecting critical regimes.
\adasp's first goal is to identify critical regimes efficiently.
Our experiments, as discussed previously (Figure~\ref{fig:critical_compare}), reveal that critical regimes can be identified by detecting the rate of change in gradient norms without using the computationally expensive technique of \cite{jastrzebski2018on, Jastrzebski2020The, keskar2016large}, where eigenvalues of the Hessian are used to detect critical regimes.  
% Shown in Figure~\ref{fig:2} are our experimental results. 
% blah blah.
This leads us to propose the following simple way to detect critical regimes:
\[
\frac{\big\lvert\norm{\Delta_{\text{old}}} - \norm{\Delta_\text{curr}} \big \rvert}{\norm{\Delta_\text{old}}} \geq \eta,
\]
where $\Delta_\text{curr}$ and  $\Delta_\text{prev}$, denotes the accumulated gradient in the current epoch and some previous epoch respectively, and $\eta$ is the threshold used to declare critical regimes.
We set $\eta = 0.5$ in all of our experiments.
For simplicity and usability, \adasp\ only switches between two levels of compression levels: $\ell_\text{low}$  and $\ell_\text{high}$.
Once \adasp\ detects critical regimes, it sets the compression level as $\ell_\text{low}$ to avoid an undesirable drop in accuracy.
Based on our observation critical regimes also almost always occur after learning rate decay, therefore we let \adasp\ declare critical regime after every learning rate decay.
If \adasp\ detects that the critical phase ends, it changes the compression level to $\ell_\text{high}$ to save communication cost.
%, since we have observed that this does not affect the final performance.
This procedure is summarized in Algorithm~\ref{alg:adasparse}.

We remark that \adasp\ operates at the granularity of the gradient compressor being used.
For instance, \powersgd\ approximates the gradients of each layer independently, so \adasp\ will also operate at each layer independently and provide a suitable compression ratio for each layer in an adaptive manner during training. While Batch size scheduling operates at the whole model so \adasp\ looks at the gradient of whole model and chooses a suitable batch size.


\noindent{\textbf{Computational and memory overhead:}}
\adasp\ accumulates gradients of each layer during the backward pass. After each epoch, norms are calculated, creating $\norm{\nabla_{curr}}$. Once the compression ratio is chosen $\norm{\nabla_{curr}}$ becomes $\norm{\nabla_{old}}$. Thus requiring only size of the model(47 MB in ResNet-18) and a few float values worth of storage. Also \adasp\ only uses the ratio between previous and current gradient norms to detect critical regimes. This allows \adasp{} to be easily integrated in a training job where gradients are already calculated, thus making the computational overhead negligible.
% pipeline Note that the
% (iii) \noindent\textbf{Better usability:}
% Choosing two compression ratios could be easier for users than choosing one compression level to use throughout training. Because it is easy to  guess a low compression level which gives good results and a high compression ratio which corresponds to a desired level of communication efficiency. 
% Thus, we believe \adasp\ at least does not increase the effort spent in hyper-parameter tuning if not reduce it.  Also, in all our experiments we find that \adasp\  does not require any change in other hyper-parameters \eg, batch size, learning rate, etc.  

% Note that \adasp\ requires the following parameters to be specified. 
% \begin{itemize}[topsep=0pt,leftmargin=2.5mm]
%     \item $\eta$: if the relative change in the gradient norm is larger than this threshold, we declare training to be in a critical regime and switch to the low compression mode. We use a constant value of 0.5 in all our experiments.
%     %\item \textsc{switch\_freq}: it determines the frequency of the change in the compression ratio. Which ends up effecting how frequently \adasp\ is invoked in the main training loop. \shivaram{not clear where this is used. current algorithm 1 doesn't have this?}
%     \item $\ell_\text{low}$  and $\ell_\text{high}$: low and high compression levels to be used. 
% \end{itemize}

%\adasp\ is invoked during training at every \textsc{switch\_freq} epoch in distributed training.

%\input{Tables/adasparse_param}
%\adasp\ operates at the granularity of the gradient compressor being used. For ex- \powersgd\ approximates the gradients of each layer independently, so \adasp\ will also operate at each layer independently and provide a suitable compression ratio accordingly.\shivaram{not clear yet why this granularity matters. maybe move this to after describing the algorithm?}

% \paragraph{Motivation:}
% \adasp\ was primarily motivated from recent work about critical regimes in neural network and behaviour of SGD in these regimes. 
% %
% We empirically observed that keeping lower compression only in these critical regimes was enough to get accuracy close to using low compression overall.
% %
% Observing the gradient norms we also noticed that these critical regimes also corresponded to rapid change in the norm of the gradient, and unlike previous work we observed that there are multiple of these critical regimes(atleast 2). In later phases of the training these critical regimes are followed by decay in learning rate. These two observations allowed us to propose \adasp\ as stated in Algorithm~\ref{alg:adasparse}. \shivaram{this seems to be repeating the intro? maybe describe in words what the algorithm is doing here? e.g., what are its inputs, what is the internal logic etc.}
%

\begin{algorithm}[tb]
\caption{\adasp}
\label{alg:adasparse}
\begin{algorithmic}
    \STATE {\bfseries HyperParameters:}compression levels \{$\ell_\text{low}$, $\ell_\text{high}$\} and detection threshold $\eta$
    \STATE {\bfseries Input:} {accumulated gradients in the current epoch ($\Delta_\text{curr}$) and in the previous epoch ($\Delta_\text{prev}$)}
    \STATE {\bfseries Input:} {learning rate of the current epoch ($\gamma_\text{curr}$) and of the next epoch ($\gamma_\text{next}$)}
    \STATE {\bfseries Output:} {compression ratio to use $\ell$}
    \IF{$\sfrac{\lvert\norm{\Delta_\text{prev}} - \norm{\Delta_\text{curr}}\rvert}{\norm{\Delta_\text{prev}}} \geq \eta$ or $\gamma_{next} < \gamma_{curr}$} %\label{ln:compare} \Comment{critical regime is detected}
        \STATE \textbf{return} $\ell_\text{low}$
    % \ElsIf{} \Comment{Training is in a critical regime}
    %     \State \textbf{return} $\ell_\text{low}$
    % 
    \ELSE
        \STATE \textbf{return} $\ell_\text{high}$
    % \EndIf
    \ENDIF
 \end{algorithmic}
\end{algorithm}
%
% \paragraph{Hyper-Parameters:}%introduced by \adasp\:}


% First is the Gradient Change Threshold \textsc{change\_thresh}, 

% . Second hyper-parameter is the the switching frequency \textsc{switch\_freq}, as seen in Algorithm~\ref{alg:dist_training} on Line~\ref{ln:dist_training:switch_freq} dictates how frequently do we want to change the compression ratio. The other two parameters are the two different low  and high compression(\lc\ and  \hc\ ) ratios to be used. 


%\adasp\ automatically switches between low and high compression ratio, while not harming the generalization performance of the model. 


%\shivaram{this is ok but seems secondary as an argument. i'd move it down or remove it}
% We first argue that 

% \paragraph{Operation}
% \adasp\ can be used with any gradient compression scheme. \adasp\ takes in accumulated gradient on all the samples from the latest epoch ($\Delta_\text{curr}$) and previous epoch ($\Delta_\text{prev}$). \eg, if the current epoch is 20 and we want to choose a new compression ratio every 10 epochs, then \adasp\ will require accumulated gradients on all minibatches in epoch 10 and epoch 20. It also requires the current learning rate ($\gamma_\text{curr}$) and the learning rate expected be used in next epoch ($\gamma_\text{next}$). If there is going to be a decay in learning rate \textit{i.e.}, $\gamma_{next} < \gamma_{curr}$, \adasp\ then picks a low compression ratio \lc. Otherwise, we use the gradient norms as described before to derive the compression ratio.
%otherwise it calculates the rate of change of gradient norm and if the rate of change is larger than Gradient Change Threshold (\textsc{change\_thresh})  it is deemed a critical regime and usage of low compression is suggested. Otherwise \adasp\ suggest to use high compression. 
%\ie \adasp\ will keep track of gradients for each layer separately to provide different compression ratios.



% \paragraph{Computation overhead:}
% Distributed training using \adasp\ is described in Algorithm~\ref{alg:dist_training}. 
% We have designed \adasp\ to have negligible computation requirements. 

%

% \begin{algorithm}
%     \caption{Distributed Training Using \adasp}
%     \label{alg:dist_training}
%     \begin{algorithmic}[1]
%     \Hyperparameters{learning rate $\alpha$, Gradient Compressor \textsc{GC}, Optimizer \textsc{OPT}, Epochs }
%     \Hyperparameters{low compression ratio \lc, high compression ratio}
%     \Hyperparameters{switch frequency \textsc{switch\_freq}, }
%     \Initialize{Model Parameters $x\in \R^d$, replicated across all nodes}
%     \Initialize{\textsc{OPT} with $\alpha$}
%     \Initialize{\textsc{GC} with $\lc$}
%     \State $epoch\gets 0$
%     \State $\textsc{C} \gets \lc$ \Comment{Bootstrap \adasp with \lc}
%     \State $grad_{old} \gets 0$ 
%     \State $grad_{curr} \gets 0$
%     \While{$epoch \leq Epochs$}
%     \At{each node $n=1, \ldots, N$}
%     \For {each minibatch $m=0,\ldots$}
%     \State {Compute stochastic gradient $\Delta_n\in \R^d$ }
%     \If {$epoch \bmod \textsc{switch\_freq} = 0$}
%     \State $grad_{curr} \gets grad_{curr} + \Delta_n$ \label{alg:ln:share}
%     \EndIf
%     \State  $\cC(\Delta_n) \gets \textsc{GC}.Compress(\Delta_n)$
%     \State  $\cC(\Delta) \gets \textsc{Aggregate}(\cC(\Delta_1), \ldots, \cC(\Delta_n))$
%     \State $\Delta \gets \textsc{GC}.DeCompress(\Delta)$
%     \State $\textsc{OPT}.Update(x,\Delta,\alpha)$ \Comment{Update Model Parameters}
%     \EndFor
%     \If{$epoch \bmod \textsc{switch\_freq} = 0$} \label{ln:dist_training:switch_freq}
%         \At {node, n=1} \Comment{Choose the first node}
%             \State{$\textsc{C} \gets \adasp$} \Comment{Use \adasp\ for to get new compression ratio}
%             \State{$\textsc{Broadcast(C)}$}
%         \EndAt
%     \State $\textsc{GC}.Reinitialize(C)$ \Comment{Reinitialize with new Compression Ratio}
%     \State{$grad_{old} \gets grad_{curr}$}
%     \State {$grad_{curr} \gets 0$}
%     \EndIf
%     \EndAt
%     \State $epoch \gets epoch +1$
%     \EndWhile
%     \end{algorithmic}
% \end{algorithm}


==> commands.tex <==
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
% \usepackage[bookmarks=false]{hyperref}   
\usepackage{url}            
\usepackage{booktabs}       
\usepackage{amsfonts,fullpage}       
\usepackage{nicefrac}       
\usepackage{microtype} 
\usepackage{wrapfig}
\usepackage{color}
\usepackage{enumitem}
\usepackage{graphicx}
\usepackage{amsmath,amssymb}
\usepackage{amsthm}
\usepackage{bigstrut}
\usepackage{float}
\usepackage{caption}
\usepackage[ruled]{algorithm2e}
\usepackage{mathtools}
\usepackage{subfigure}
\usepackage{booktabs}
\usepackage{authblk}

\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem*{notation}{Notation}
\newtheorem{remark}{Remark}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{example}{Example}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{conjecture}{Conjecture}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem*{conjecturess}{Conjecture}
\newtheorem*{propositionss}{Proposition}
\newtheorem{asm}{Assumption}
\newtheorem{question}{Question}[]

\newcommand{\eq}[1]{(\ref{eq:#1})}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\sign}{sign}
\DeclareMathOperator*{\Ber}{Ber}
\DeclareMathOperator*{\tr}{tr}
\DeclareMathOperator*{\vecc}{vec}
\DeclareMathOperator*{\Var}{Var}

\newcommand{\PP}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\cmp}{\mathbb{C}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\atomsgd}{\textsc{Atomo}}
\newcommand{\eg}{\textit{e.g.}}
\newcommand{\ie}{\textit{i.e.}, }

\newcommand\Tstrut{\rule{0pt}{1.5\normalbaselineskip}}
\newcommand\Bstrut{\rule[-1.0\normalbaselineskip]{0pt}{0pt}} 

\usepackage{color}
\definecolor{myblue}{rgb}{.8, .8, 1}

\usepackage{empheq}

\newlength\mytemplen
\newsavebox\mytempbox

\makeatletter
\newcommand\mybluebox{%
	\@ifnextchar[%]
	{\@mybluebox}%
	{\@mybluebox[0pt]}}

\def\@mybluebox[#1]{%
	\@ifnextchar[%]
	{\@@mybluebox[#1]}%
	{\@@mybluebox[#1][0pt]}}

\def\@@mybluebox[#1][#2]#3{
	\sbox\mytempbox{#3}%
	\mytemplen\ht\mytempbox
	\advance\mytemplen #1\relax
	\ht\mytempbox\mytemplen
	\mytemplen\dp\mytempbox
	\advance\mytemplen #2\relax
	\dp\mytempbox\mytemplen
	\colorbox{myblue}{\hspace{1em}\usebox{\mytempbox}\hspace{1em}}}

\makeatother


\usepackage[most]{tcolorbox}

\newtcbox{\mymath}[1][]{%
	nobeforeafter, math upper, tcbox raise base,
	enhanced, colframe=blue!30!black,
	colback=blue!30, boxrule=1pt,
	#1}

%%%%

% Single-line affiliation
% \makeatletter
% \renewcommand\AB@affilsepx{, \protect\Affilfont}
% \makeatother



==> fancyhdr.tex <==
% fancyhdr.sty version 3.2
% Fancy headers and footers for LaTeX.
% Piet van Oostrum, 
% Dept of Computer and Information Sciences, University of Utrecht,
% Padualaan 14, P.O. Box 80.089, 3508 TB Utrecht, The Netherlands
% Telephone: +31 30 2532180. Email: piet@cs.uu.nl
% ========================================================================
% LICENCE:
% This file may be distributed under the terms of the LaTeX Project Public
% License, as described in lppl.txt in the base LaTeX distribution.
% Either version 1 or, at your option, any later version.
% ========================================================================
% MODIFICATION HISTORY:
% Sep 16, 1994
% version 1.4: Correction for use with \reversemargin
% Sep 29, 1994:
% version 1.5: Added the \iftopfloat, \ifbotfloat and \iffloatpage commands
% Oct 4, 1994:
% version 1.6: Reset single spacing in headers/footers for use with
% setspace.sty or doublespace.sty
% Oct 4, 1994:
% version 1.7: changed \let\@mkboth\markboth to
% \def\@mkboth{\protect\markboth} to make it more robust
% Dec 5, 1994:
% version 1.8: corrections for amsbook/amsart: define \@chapapp and (more
% importantly) use the \chapter/sectionmark definitions from ps@headings if
% they exist (which should be true for all standard classes).
% May 31, 1995:
% version 1.9: The proposed \renewcommand{\headrulewidth}{\iffloatpage...
% construction in the doc did not work properly with the fancyplain style. 
% June 1, 1995:
% version 1.91: The definition of \@mkboth wasn't restored on subsequent
% \pagestyle{fancy}'s.
% June 1, 1995:
% version 1.92: The sequence \pagestyle{fancyplain} \pagestyle{plain}
% \pagestyle{fancy} would erroneously select the plain version.
% June 1, 1995:
% version 1.93: \fancypagestyle command added.
% Dec 11, 1995:
% version 1.94: suggested by Conrad Hughes <chughes@maths.tcd.ie>
% CJCH, Dec 11, 1995: added \footruleskip to allow control over footrule
% position (old hardcoded value of .3\normalbaselineskip is far too high
% when used with very small footer fonts).
% Jan 31, 1996:
% version 1.95: call \@normalsize in the reset code if that is defined,
% otherwise \normalsize.
% this is to solve a problem with ucthesis.cls, as this doesn't
% define \@currsize. Unfortunately for latex209 calling \normalsize doesn't
% work as this is optimized to do very little, so there \@normalsize should
% be called. Hopefully this code works for all versions of LaTeX known to
% mankind.  
% April 25, 1996:
% version 1.96: initialize \headwidth to a magic (negative) value to catch
% most common cases that people change it before calling \pagestyle{fancy}.
% Note it can't be initialized when reading in this file, because
% \textwidth could be changed afterwards. This is quite probable.
% We also switch to \MakeUppercase rather than \uppercase and introduce a
% \nouppercase command for use in headers. and footers.
% May 3, 1996:
% version 1.97: Two changes:
% 1. Undo the change in version 1.8 (using the pagestyle{headings} defaults
% for the chapter and section marks. The current version of amsbook and
% amsart classes don't seem to need them anymore. Moreover the standard
% latex classes don't use \markboth if twoside isn't selected, and this is
% confusing as \leftmark doesn't work as expected.
% 2. include a call to \ps@empty in ps@@fancy. This is to solve a problem
% in the amsbook and amsart classes, that make global changes to \topskip,
% which are reset in \ps@empty. Hopefully this doesn't break other things.
% May 7, 1996:
% version 1.98:
% Added % after the line  \def\nouppercase
% May 7, 1996:
% version 1.99: This is the alpha version of fancyhdr 2.0
% Introduced the new commands \fancyhead, \fancyfoot, and \fancyhf.
% Changed \headrulewidth, \footrulewidth, \footruleskip to
% macros rather than length parameters, In this way they can be
% conditionalized and they don't consume length registers. There is no need
% to have them as length registers unless you want to do calculations with
% them, which is unlikely. Note that this may make some uses of them
% incompatible (i.e. if you have a file that uses \setlength or \xxxx=)
% May 10, 1996:
% version 1.99a:
% Added a few more % signs
% May 10, 1996:
% version 1.99b:
% Changed the syntax of \f@nfor to be resistent to catcode changes of :=
% Removed the [1] from the defs of \lhead etc. because the parameter is
% consumed by the \@[xy]lhead etc. macros.
% June 24, 1997:
% version 1.99c:
% corrected \nouppercase to also include the protected form of \MakeUppercase
% \global added to manipulation of \headwidth.
% \iffootnote command added.
% Some comments added about \@fancyhead and \@fancyfoot.
% Aug 24, 1998
% version 1.99d
% Changed the default \ps@empty to \ps@@empty in order to allow
% \fancypagestyle{empty} redefinition.
% Oct 11, 2000
% version 2.0
% Added LPPL license clause.
%
% A check for \headheight is added. An errormessage is given (once) if the
% header is too large. Empty headers don't generate the error even if
% \headheight is very small or even 0pt. 
% Warning added for the use of 'E' option when twoside option is not used.
% In this case the 'E' fields will never be used.
%
% Mar 10, 2002
% version 2.1beta
% New command: \fancyhfoffset[place]{length}
% defines offsets to be applied to the header/footer to let it stick into
% the margins (if length > 0).
% place is like in fancyhead, except that only E,O,L,R can be used.
% This replaces the old calculation based on \headwidth and the marginpar
% area.
% \headwidth will be dynamically calculated in the headers/footers when
% this is used.
%
% Mar 26, 2002
% version 2.1beta2
% \fancyhfoffset now also takes h,f as possible letters in the argument to
% allow the header and footer widths to be different.
% New commands \fancyheadoffset and \fancyfootoffset added comparable to
% \fancyhead and \fancyfoot.
% Errormessages and warnings have been made more informative.
%
% Dec 9, 2002
% version 2.1
% The defaults for \footrulewidth, \plainheadrulewidth and
% \plainfootrulewidth are changed from \z@skip to 0pt. In this way when
% someone inadvertantly uses \setlength to change any of these, the value
% of \z@skip will not be changed, rather an errormessage will be given.

% March 3, 2004
% Release of version 3.0

% Oct 7, 2004
% version 3.1
% Added '\endlinechar=13' to \fancy@reset to prevent problems with
% includegraphics in header when verbatiminput is active.

% March 22, 2005
% version 3.2
% reset \everypar (the real one) in \fancy@reset because spanish.ldf does
% strange things with \everypar between << and >>.

\def\ifancy@mpty#1{\def\temp@a{#1}\ifx\temp@a\@empty}

\def\fancy@def#1#2{\ifancy@mpty{#2}\fancy@gbl\def#1{\leavevmode}\else
                                   \fancy@gbl\def#1{#2\strut}\fi}

\let\fancy@gbl\global

\def\@fancyerrmsg#1{%
        \ifx\PackageError\undefined
        \errmessage{#1}\else
        \PackageError{Fancyhdr}{#1}{}\fi}
\def\@fancywarning#1{%
        \ifx\PackageWarning\undefined
        \errmessage{#1}\else
        \PackageWarning{Fancyhdr}{#1}{}\fi}

% Usage: \@forc \var{charstring}{command to be executed for each char}
% This is similar to LaTeX's \@tfor, but expands the charstring.

\def\@forc#1#2#3{\expandafter\f@rc\expandafter#1\expandafter{#2}{#3}}
\def\f@rc#1#2#3{\def\temp@ty{#2}\ifx\@empty\temp@ty\else
                                    \f@@rc#1#2\f@@rc{#3}\fi}
\def\f@@rc#1#2#3\f@@rc#4{\def#1{#2}#4\f@rc#1{#3}{#4}}

% Usage: \f@nfor\name:=list\do{body}
% Like LaTeX's \@for but an empty list is treated as a list with an empty
% element

\newcommand{\f@nfor}[3]{\edef\@fortmp{#2}%
    \expandafter\@forloop#2,\@nil,\@nil\@@#1{#3}}

% Usage: \def@ult \cs{defaults}{argument}
% sets \cs to the characters from defaults appearing in argument
% or defaults if it would be empty. All characters are lowercased.

\newcommand\def@ult[3]{%
    \edef\temp@a{\lowercase{\edef\noexpand\temp@a{#3}}}\temp@a
    \def#1{}%
    \@forc\tmpf@ra{#2}%
        {\expandafter\if@in\tmpf@ra\temp@a{\edef#1{#1\tmpf@ra}}{}}%
    \ifx\@empty#1\def#1{#2}\fi}
% 
% \if@in <char><set><truecase><falsecase>
%
\newcommand{\if@in}[4]{%
    \edef\temp@a{#2}\def\temp@b##1#1##2\temp@b{\def\temp@b{##1}}%
    \expandafter\temp@b#2#1\temp@b\ifx\temp@a\temp@b #4\else #3\fi}

\newcommand{\fancyhead}{\@ifnextchar[{\f@ncyhf\fancyhead h}%
                                     {\f@ncyhf\fancyhead h[]}}
\newcommand{\fancyfoot}{\@ifnextchar[{\f@ncyhf\fancyfoot f}%
                                     {\f@ncyhf\fancyfoot f[]}}
\newcommand{\fancyhf}{\@ifnextchar[{\f@ncyhf\fancyhf{}}%
                                   {\f@ncyhf\fancyhf{}[]}}

% New commands for offsets added

\newcommand{\fancyheadoffset}{\@ifnextchar[{\f@ncyhfoffs\fancyheadoffset h}%
                                           {\f@ncyhfoffs\fancyheadoffset h[]}}
\newcommand{\fancyfootoffset}{\@ifnextchar[{\f@ncyhfoffs\fancyfootoffset f}%
                                           {\f@ncyhfoffs\fancyfootoffset f[]}}
\newcommand{\fancyhfoffset}{\@ifnextchar[{\f@ncyhfoffs\fancyhfoffset{}}%
                                         {\f@ncyhfoffs\fancyhfoffset{}[]}}

% The header and footer fields are stored in command sequences with
% names of the form: \f@ncy<x><y><z> with <x> for [eo], <y> from [lcr]
% and <z> from [hf].

\def\f@ncyhf#1#2[#3]#4{%
    \def\temp@c{}%
    \@forc\tmpf@ra{#3}%
        {\expandafter\if@in\tmpf@ra{eolcrhf,EOLCRHF}%
            {}{\edef\temp@c{\temp@c\tmpf@ra}}}%
    \ifx\@empty\temp@c\else
        \@fancyerrmsg{Illegal char `\temp@c' in \string#1 argument:
          [#3]}%
    \fi
    \f@nfor\temp@c{#3}%
        {\def@ult\f@@@eo{eo}\temp@c
         \if@twoside\else
           \if\f@@@eo e\@fancywarning
             {\string#1's `E' option without twoside option is useless}\fi\fi
         \def@ult\f@@@lcr{lcr}\temp@c
         \def@ult\f@@@hf{hf}{#2\temp@c}%
         \@forc\f@@eo\f@@@eo
             {\@forc\f@@lcr\f@@@lcr
                 {\@forc\f@@hf\f@@@hf
                     {\expandafter\fancy@def\csname
                      f@ncy\f@@eo\f@@lcr\f@@hf\endcsname
                      {#4}}}}}}

\def\f@ncyhfoffs#1#2[#3]#4{%
    \def\temp@c{}%
    \@forc\tmpf@ra{#3}%
        {\expandafter\if@in\tmpf@ra{eolrhf,EOLRHF}%
            {}{\edef\temp@c{\temp@c\tmpf@ra}}}%
    \ifx\@empty\temp@c\else
        \@fancyerrmsg{Illegal char `\temp@c' in \string#1 argument:
          [#3]}%
    \fi
    \f@nfor\temp@c{#3}%
        {\def@ult\f@@@eo{eo}\temp@c
         \if@twoside\else
           \if\f@@@eo e\@fancywarning
             {\string#1's `E' option without twoside option is useless}\fi\fi
         \def@ult\f@@@lcr{lr}\temp@c
         \def@ult\f@@@hf{hf}{#2\temp@c}%
         \@forc\f@@eo\f@@@eo
             {\@forc\f@@lcr\f@@@lcr
                 {\@forc\f@@hf\f@@@hf
                     {\expandafter\setlength\csname
                      f@ncyO@\f@@eo\f@@lcr\f@@hf\endcsname
                      {#4}}}}}%
     \fancy@setoffs}

% Fancyheadings version 1 commands. These are more or less deprecated,
% but they continue to work.

\newcommand{\lhead}{\@ifnextchar[{\@xlhead}{\@ylhead}}
\def\@xlhead[#1]#2{\fancy@def\f@ncyelh{#1}\fancy@def\f@ncyolh{#2}}
\def\@ylhead#1{\fancy@def\f@ncyelh{#1}\fancy@def\f@ncyolh{#1}}

\newcommand{\chead}{\@ifnextchar[{\@xchead}{\@ychead}}
\def\@xchead[#1]#2{\fancy@def\f@ncyech{#1}\fancy@def\f@ncyoch{#2}}
\def\@ychead#1{\fancy@def\f@ncyech{#1}\fancy@def\f@ncyoch{#1}}

\newcommand{\rhead}{\@ifnextchar[{\@xrhead}{\@yrhead}}
\def\@xrhead[#1]#2{\fancy@def\f@ncyerh{#1}\fancy@def\f@ncyorh{#2}}
\def\@yrhead#1{\fancy@def\f@ncyerh{#1}\fancy@def\f@ncyorh{#1}}

\newcommand{\lfoot}{\@ifnextchar[{\@xlfoot}{\@ylfoot}}
\def\@xlfoot[#1]#2{\fancy@def\f@ncyelf{#1}\fancy@def\f@ncyolf{#2}}
\def\@ylfoot#1{\fancy@def\f@ncyelf{#1}\fancy@def\f@ncyolf{#1}}

\newcommand{\cfoot}{\@ifnextchar[{\@xcfoot}{\@ycfoot}}
\def\@xcfoot[#1]#2{\fancy@def\f@ncyecf{#1}\fancy@def\f@ncyocf{#2}}
\def\@ycfoot#1{\fancy@def\f@ncyecf{#1}\fancy@def\f@ncyocf{#1}}

\newcommand{\rfoot}{\@ifnextchar[{\@xrfoot}{\@yrfoot}}
\def\@xrfoot[#1]#2{\fancy@def\f@ncyerf{#1}\fancy@def\f@ncyorf{#2}}
\def\@yrfoot#1{\fancy@def\f@ncyerf{#1}\fancy@def\f@ncyorf{#1}}

\newlength{\fancy@headwidth}
\let\headwidth\fancy@headwidth
\newlength{\f@ncyO@elh}
\newlength{\f@ncyO@erh}
\newlength{\f@ncyO@olh}
\newlength{\f@ncyO@orh}
\newlength{\f@ncyO@elf}
\newlength{\f@ncyO@erf}
\newlength{\f@ncyO@olf}
\newlength{\f@ncyO@orf}
\newcommand{\headrulewidth}{0.4pt}
\newcommand{\footrulewidth}{0pt}
\newcommand{\footruleskip}{.3\normalbaselineskip}

% Fancyplain stuff shouldn't be used anymore (rather
% \fancypagestyle{plain} should be used), but it must be present for
% compatibility reasons.

\newcommand{\plainheadrulewidth}{0pt}
\newcommand{\plainfootrulewidth}{0pt}
\newif\if@fancyplain \@fancyplainfalse
\def\fancyplain#1#2{\if@fancyplain#1\else#2\fi}

\headwidth=-123456789sp %magic constant

% Command to reset various things in the headers:
% a.o.  single spacing (taken from setspace.sty)
% and the catcode of ^^M (so that epsf files in the header work if a
% verbatim crosses a page boundary)
% It also defines a \nouppercase command that disables \uppercase and
% \Makeuppercase. It can only be used in the headers and footers.
\let\fnch@everypar\everypar% save real \everypar because of spanish.ldf
\def\fancy@reset{\fnch@everypar{}\restorecr\endlinechar=13
 \def\baselinestretch{1}%
 \def\nouppercase##1{{\let\uppercase\relax\let\MakeUppercase\relax
     \expandafter\let\csname MakeUppercase \endcsname\relax##1}}%
 \ifx\undefined\@newbaseline% NFSS not present; 2.09 or 2e
   \ifx\@normalsize\undefined \normalsize % for ucthesis.cls
   \else \@normalsize \fi
 \else% NFSS (2.09) present
  \@newbaseline%
 \fi}

% Initialization of the head and foot text.

% The default values still contain \fancyplain for compatibility.
\fancyhf{} % clear all
% lefthead empty on ``plain'' pages, \rightmark on even, \leftmark on odd pages
% evenhead empty on ``plain'' pages, \leftmark on even, \rightmark on odd pages
\if@twoside
  \fancyhead[el,or]{\fancyplain{}{\sl\rightmark}}
  \fancyhead[er,ol]{\fancyplain{}{\sl\leftmark}}
\else
  \fancyhead[l]{\fancyplain{}{\sl\rightmark}}
  \fancyhead[r]{\fancyplain{}{\sl\leftmark}}
\fi
\fancyfoot[c]{\rm\thepage} % page number

% Use box 0 as a temp box and dimen 0 as temp dimen. 
% This can be done, because this code will always
% be used inside another box, and therefore the changes are local.

\def\@fancyvbox#1#2{\setbox0\vbox{#2}\ifdim\ht0>#1\@fancywarning
  {\string#1 is too small (\the#1): ^^J Make it at least \the\ht0.^^J
    We now make it that large for the rest of the document.^^J
    This may cause the page layout to be inconsistent, however\@gobble}%
  \dimen0=#1\global\setlength{#1}{\ht0}\ht0=\dimen0\fi
  \box0}

% Put together a header or footer given the left, center and
% right text, fillers at left and right and a rule.
% The \lap commands put the text into an hbox of zero size,
% so overlapping text does not generate an errormessage.
% These macros have 5 parameters:
% 1. LEFTSIDE BEARING % This determines at which side the header will stick
%    out. When \fancyhfoffset is used this calculates \headwidth, otherwise
%    it is \hss or \relax (after expansion).
% 2. \f@ncyolh, \f@ncyelh, \f@ncyolf or \f@ncyelf. This is the left component.
% 3. \f@ncyoch, \f@ncyech, \f@ncyocf or \f@ncyecf. This is the middle comp.
% 4. \f@ncyorh, \f@ncyerh, \f@ncyorf or \f@ncyerf. This is the right component.
% 5. RIGHTSIDE BEARING. This is always \relax or \hss (after expansion).

\def\@fancyhead#1#2#3#4#5{#1\hbox to\headwidth{\fancy@reset
  \@fancyvbox\headheight{\hbox
    {\rlap{\parbox[b]{\headwidth}{\raggedright#2}}\hfill
      \parbox[b]{\headwidth}{\centering#3}\hfill
      \llap{\parbox[b]{\headwidth}{\raggedleft#4}}}\headrule}}#5}

\def\@fancyfoot#1#2#3#4#5{#1\hbox to\headwidth{\fancy@reset
    \@fancyvbox\footskip{\footrule
      \hbox{\rlap{\parbox[t]{\headwidth}{\raggedright#2}}\hfill
        \parbox[t]{\headwidth}{\centering#3}\hfill
        \llap{\parbox[t]{\headwidth}{\raggedleft#4}}}}}#5}

\def\headrule{{\if@fancyplain\let\headrulewidth\plainheadrulewidth\fi
    \hrule\@height\headrulewidth\@width\headwidth \vskip-\headrulewidth}}

\def\footrule{{\if@fancyplain\let\footrulewidth\plainfootrulewidth\fi
    \vskip-\footruleskip\vskip-\footrulewidth
    \hrule\@width\headwidth\@height\footrulewidth\vskip\footruleskip}}

\def\ps@fancy{%
\@ifundefined{@chapapp}{\let\@chapapp\chaptername}{}%for amsbook
%
% Define \MakeUppercase for old LaTeXen.
% Note: we used \def rather than \let, so that \let\uppercase\relax (from
% the version 1 documentation) will still work.
%
\@ifundefined{MakeUppercase}{\def\MakeUppercase{\uppercase}}{}%
\@ifundefined{chapter}{\def\sectionmark##1{\markboth
{\MakeUppercase{\ifnum \c@secnumdepth>\z@
 \thesection\hskip 1em\relax \fi ##1}}{}}%
\def\subsectionmark##1{\markright {\ifnum \c@secnumdepth >\@ne
 \thesubsection\hskip 1em\relax \fi ##1}}}%
{\def\chaptermark##1{\markboth {\MakeUppercase{\ifnum \c@secnumdepth>\m@ne
 \@chapapp\ \thechapter. \ \fi ##1}}{}}%
\def\sectionmark##1{\markright{\MakeUppercase{\ifnum \c@secnumdepth >\z@
 \thesection. \ \fi ##1}}}}%
%\csname ps@headings\endcsname % use \ps@headings defaults if they exist
\ps@@fancy
\gdef\ps@fancy{\@fancyplainfalse\ps@@fancy}%
% Initialize \headwidth if the user didn't
%
\ifdim\headwidth<0sp
%
% This catches the case that \headwidth hasn't been initialized and the
% case that the user added something to \headwidth in the expectation that
% it was initialized to \textwidth. We compensate this now. This loses if
% the user intended to multiply it by a factor. But that case is more
% likely done by saying something like \headwidth=1.2\textwidth. 
% The doc says you have to change \headwidth after the first call to
% \pagestyle{fancy}. This code is just to catch the most common cases were
% that requirement is violated.
%
    \global\advance\headwidth123456789sp\global\advance\headwidth\textwidth
\fi}
\def\ps@fancyplain{\ps@fancy \let\ps@plain\ps@plain@fancy}
\def\ps@plain@fancy{\@fancyplaintrue\ps@@fancy}
\let\ps@@empty\ps@empty
\def\ps@@fancy{%
\ps@@empty % This is for amsbook/amsart, which do strange things with \topskip
\def\@mkboth{\protect\markboth}%
\def\@oddhead{\@fancyhead\fancy@Oolh\f@ncyolh\f@ncyoch\f@ncyorh\fancy@Oorh}%
\def\@oddfoot{\@fancyfoot\fancy@Oolf\f@ncyolf\f@ncyocf\f@ncyorf\fancy@Oorf}%
\def\@evenhead{\@fancyhead\fancy@Oelh\f@ncyelh\f@ncyech\f@ncyerh\fancy@Oerh}%
\def\@evenfoot{\@fancyfoot\fancy@Oelf\f@ncyelf\f@ncyecf\f@ncyerf\fancy@Oerf}%
}
% Default definitions for compatibility mode:
% These cause the header/footer to take the defined \headwidth as width
% And to shift in the direction of the marginpar area

\def\fancy@Oolh{\if@reversemargin\hss\else\relax\fi}
\def\fancy@Oorh{\if@reversemargin\relax\else\hss\fi}
\let\fancy@Oelh\fancy@Oorh
\let\fancy@Oerh\fancy@Oolh

\let\fancy@Oolf\fancy@Oolh
\let\fancy@Oorf\fancy@Oorh
\let\fancy@Oelf\fancy@Oelh
\let\fancy@Oerf\fancy@Oerh

% New definitions for the use of \fancyhfoffset
% These calculate the \headwidth from \textwidth and the specified offsets.

\def\fancy@offsolh{\headwidth=\textwidth\advance\headwidth\f@ncyO@olh
                   \advance\headwidth\f@ncyO@orh\hskip-\f@ncyO@olh}
\def\fancy@offselh{\headwidth=\textwidth\advance\headwidth\f@ncyO@elh
                   \advance\headwidth\f@ncyO@erh\hskip-\f@ncyO@elh}

\def\fancy@offsolf{\headwidth=\textwidth\advance\headwidth\f@ncyO@olf
                   \advance\headwidth\f@ncyO@orf\hskip-\f@ncyO@olf}
\def\fancy@offself{\headwidth=\textwidth\advance\headwidth\f@ncyO@elf
                   \advance\headwidth\f@ncyO@erf\hskip-\f@ncyO@elf}

\def\fancy@setoffs{%
% Just in case \let\headwidth\textwidth was used
  \fancy@gbl\let\headwidth\fancy@headwidth
  \fancy@gbl\let\fancy@Oolh\fancy@offsolh
  \fancy@gbl\let\fancy@Oelh\fancy@offselh
  \fancy@gbl\let\fancy@Oorh\hss
  \fancy@gbl\let\fancy@Oerh\hss
  \fancy@gbl\let\fancy@Oolf\fancy@offsolf
  \fancy@gbl\let\fancy@Oelf\fancy@offself
  \fancy@gbl\let\fancy@Oorf\hss
  \fancy@gbl\let\fancy@Oerf\hss}

\newif\iffootnote
\let\latex@makecol\@makecol
\def\@makecol{\ifvoid\footins\footnotetrue\else\footnotefalse\fi
\let\topfloat\@toplist\let\botfloat\@botlist\latex@makecol}
\def\iftopfloat#1#2{\ifx\topfloat\empty #2\else #1\fi}
\def\ifbotfloat#1#2{\ifx\botfloat\empty #2\else #1\fi}
\def\iffloatpage#1#2{\if@fcolmade #1\else #2\fi}

\newcommand{\fancypagestyle}[2]{%
  \@namedef{ps@#1}{\let\fancy@gbl\relax#2\relax\ps@fancy}}


==> intro-again.tex <==
\section{Introduction}
Billion-parameter scale neural networks and the rapid increase in compute requirements for training them, has made distributed gradient-based methods a necessity. 
%
Synchronous, data-parallel training is the most widely adopted approach in this context, and requires combining per-node gradient updates every iteration~\cite{dean2012comm, iandola2016firecaffe, goyal2017accurate, shallue2018measuring}.
%(QUESTION: do we need to go a bit more detail about communication, like how much and how often)
Frequently communicating gradients of millions of parameters, across large number of nodes leads to sub-optimal scalability in distributed implementations~\cite{dean2012comm, seide20141bit, alistarh2017qsgd, dawn2019scale, luo2020plink}.
%
% overheads that cause

To alleviate these gradient communication bottlenecks, recent work has primarily focused on lossy gradient compression using a variety of techniques. 
One of the most popular ways to achieve gradient compression is low-precision training that has been heavily studied in past few years \cite{alistarh2017qsgd, seide20141bit, wen2017terngrad, bernstein2018signsgd, acharya2019distributed}.
%
Another line of work~\cite{aji2017sparse, shi2019distributed, shi2019understanding, lin2017deep} exchanges only the largest gradient coordinates. 
These methods are usually referred to as \topk\ where \textsc{K} refers to the total number of coordinates communicated per iteration. 
%
Recently, \cite{wang2018atomo, vogels2019powersgd} have shown how to perform efficient gradient compression using extremely low-rank updates.
% \powersgd\cite{vogels2019powersgd} is a practical low rank method providing end to end speedup.
 %
To alleviate the problem of bias in compressed gradients \citep{stich2018sparsified, stich2019error} utilize error feed-back that fixes biases and leads to improved convergence.
%Other work to reduce communication focus on reducing the frequency of gradient updates \cite{stich2019local, wang2020overlap}.
%Not sure if we need the local sgd stuff

% require choosing
All the proposed methods use an extra hyper-parameter which determines the compression or sparsification ratio before training begins.
%
For instance, \topk~\cite{aji2017sparse} requires choosing a hyperparamter \textsc{K} that denotes the number of large-magnitude entries that are going to be communicated in each iteration.  
%
Similarly \powersgd~\cite{vogels2019powersgd}, a low-rank approximation method, requires choosing the rank for the low rank approximation.
%
Choosing compression ratios presents a seemingly inherent trade-off between final model accuracy and per iteration communication overhead. 
%\kw{By carefully choosing compression ratios for these algortihms, one can strike a balance between the final model accuracy and the per-iteration communication overhead.}
%
For instance, training ResNet-18 on \cifart\ using \topk 10\% sparsification takes around 3.6$\times$ less wall-clock time than training using \topk 99\%, but causes around 1.5\% degradation in final accuracy.  Similar trade-offs are observed in~\cite{vogels2019powersgd, alistarh2017qsgd, wang2018atomo, aji2017sparse}.
%

This raises a fundamental question:  \textit{Is this observed trade-off fundamental?}  
In this work, we first show that such a trade-off is \emph{not} fundamental but a mere artifact of using a fixed compression rate throughout training.
In other words, if a gradient compression rate is chosen carefully, like it is done for learning rate or batch size~\cite{smith2017cyclical,Liu2020On, duchi2011adaptive, loshchilov2016sgdr, kingma2014adam, goyal2017accurate}, then  both the final model performance and communication efficiency can be improved, when compared against fixed gradient compression rate throughout training.
Figure~\ref{fig:critical_regimes_cifar100} shows an experiment where we train ResNet-18 on \cifarh, with different compression schemes.  We see that there exists an adaptive compression scheme that can significantly reduces communication while maintaining final test accuracy. 



% In other words, if one can carefully choose a gradient compression rate schedule, as we do for learning rate or batchsize~\cite{smith2017cyclical,Liu2020On, duchi2011adaptive, loshchilov2016sgdr, kingma2014adam, goyal2017accurate}, then one can indeed improve both the final model performance and communication efficiency, compared to the cases where a fixed gradient compression rate is used throughout training.


Our finding -- that there exists a communication-effective adaptive gradient compression scheme that does not hurt the final test accuracy -- is closely related to recent findings made in the deep learning literature. 
In recent work by~\citet{achille2018critical}, the authors show the existence of so-called \emph{critical regimes}, an early phase of training where adding small noise to the data can affect the regions to which training algorithms are steered to in later phases of training, often resulting in poor generalization.
This is coherent with our finding that there exist certain critical regimes where using a high gradient compression ratio can significantly affect the final test accuracy.  % as our algorithm is also based on the observation
% in which gradient compression does hurt the final generalization performance as well as \emph{non-critical regimes} in which compression does not affect much.
% We remark that our finding is consistent with recent findings made in the literature.
Furthermore, our finding is also consistent with recent findings about the effect of batch-size scheduling on the final test accuracy. 
In~\cite{goyal2017accurate, devarakonda2017adabatch}, the authors have shown that the final test accuracy is significantly impaired if large mini-batches are used in early phase of training.
Moreover, they show that the final test accuracy is not affected even when large batch size is used in later phase of training. 
This is also closely related to our finding and we show that there exists an implicit equivalence between gradient compression and large-batch training under certain conditions.  


% how one can 
While our finding implies the existence of effective adaptive compression schedules, there remain challenges in designing an adaptive compression strategy that is generic across models and compression schemes while imposing low computational overheads. 
We propose \adasp, a simple but powerful gradient compression scheduling algorithm, which can be applied to any existing distributed SGD setup with any gradient compression scheme. 
\adasp\ first identifies whether the current training regime is critical or non-critical by inspecting the change in the gradient norms, and then accordingly adjusts the gradient compression rate.
% Via extensive experiments, we first show that \adasp\ can reliably identify whether or not training is in critical regimes.
We show that \adasp\ can achieve improved communication efficiency while maintaining high generalization performance on computer vision and language modelling tasks. 
In particular, using the SOTA sparsification (\topk) and low-rank approximation methods (\powersgd), we show reduction in communication upto 3.7$\times$ and speedup upto 3.6$\times$ compared to using low compression throughout, while achieving similar accuracy. % as using low compression.





\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/accuracy_critical_regions_resnet18_cifar100.pdf}
    \caption{\small{\textbf{Effect of gradient compression in Critical Regimes when Training ResNet-18 on \cifarh:} We conduct these on a 4 Node cluster using \powersgd\ \textsc{Rank 2} (low compression) and \textsc{Rank 1} (high compression) (left) Accuracy vs Epochs, there exist a compression pattern which provides similar training accuracy as using low compression(\textsc{Rank 2}) throughout. (right) Accuracy vs Floats Communicated, this compression pattern communicates significantly less than using low compression throughout (\textsc{Rank 2}) }}
    \label{fig:critical_regimes_cifar100}
    \vspace{-0.1in}
\end{figure}


% \begin{figure}[t]
%     \begin{center}
%     \begin{subfigure}[b]{0.49\textwidth}
%         \includegraphics[width=0.9\textwidth]{Figures/accuracy_critical_regions_resnet18.pdf}
%         \caption{Effect of using different Compression Ratios in Critical Regimes on (left)accuracy vs Epochs and (right)Accuracy vs Floats communication }
%         \vspace{-0.1in}
%         \label{fig:1a}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.49\textwidth}
%         \includegraphics[width=0.9\textwidth]{Figures/accuracy_critical_regions_resnet18_cifar100.pdf}
%         \caption{Critical Regions}
%         \vspace{-0.03in}
%         \label{fig:1b}
%     \end{subfigure}
%     % \begin{subfigure}[b]{0.9\textwidth}
%     %     \includegraphics[width=0.9\textwidth]{Figures/psgd_senet_cifar10.pdf}
%     %     \caption{Cifar10, SeNet}
%     % \end{subfigure}
%     \end{center}
%     \caption{\small{\textbf{Effect of Gradient Compression in Critical Regimes when Training ResNet-18 on \cifart:} This experiment was performed for 4 Nodes (a) We show that critical regimes can be identified with rapid change in gradient norm. (b, left) Shows the effect of running \powersgd\ with different compression ratios and it's  effect on final accuracy. It can be observed that keeping \mbox{\textsc{Rank 4}} (better estimate of the gradient, lower Compression) in the critical regimes and \mbox{\textsc{Rank 1}} (poor estimate of the gradient, Higher Compression) elsewhere is sufficient to reach the same accuracy as keeping \mbox{\textsc{Rank 4}} throughout. Further keeping \mbox{\textsc{Rank 1}} in these critical regimes is detrimental to the accuracy and can not be compensated with \textsc{Rank 4} elsewhere. %To further highlight the importance of maintaining a low compression rate in these critical regimes, we also test a scheme where \mbox{\textsc{Rank 1}} is chosen only within those critical regimes, while \mbox{\textsc{Rank 4}} is used elsewhere. 
%     (b,right) Shows Accuracy vs Float communicated, even though the communication is high for using \textsc{Rank 1} in critical regimes and \textsc{Rank 4} otherwise, there is significant drop in Test Accuracy. This shows the relationship between Communication and Accuracy is not linear. \ie more Communication doesn't imply better Test Performance}}
%     \label{fig:critical_regimes}
%     \vspace{-0.26in}
% \end{figure}


%
% We employ these insights to gradient compression:
% as long as we're outside of a critical learning regime, low accuracy gradients are sufficient for training, but should be avoided once in it. We validate these insights in Figure~\ref{fig:critical_regimes}, where we show that if we over-compress gradients during these critical regimes, then test accuracy is significantly impaired.
% %
% On the other hand, we show that when compression ratios are selected conservatively to avoid impairing the training process during these critical regimes, then test error is unaffected, even if high compression is used in other regimes.
% %
% %Furthermore, we propose a simple method that identifies such critical regimes by continuously inspecting the scale of gradient norms while training . 
% {\color{red}[DP: I want to add that folks may complain here and say, how does fast gradient change relate to the literature. Can you ellaborate on this] \address{I am not aware of literature around fast gradient change i tried to look couldn't find something}}
% %

% Inspired by these observations, we propose \adasp\ an online algorithm that automatically identifies critical regimes and accordingly switches between low/high compression modes.
% %
% Unlike the computationally expensive methods of~\cite{keskar2016large, Jastrzebski2020The} where critical regimes are characterized by eigenvalues of the Hessian matrix, \adasp\ uses rate of change in gradient norm to identify critical regime.
% %
% This makes \adasp's computational overhead almost negligible.
% %TODO: Formulate the 
% %
% We evaluate training performance of \adasp\ on computer vision and language modelling tasks. 
% %

%Keeping the sparsification constant throughout training is at odds with recent work which has shown presence of critical regimes in neural network training, since one would assume that these regimes 
%
% It has been suggested that various important aspects of training occur in early phase of neural network training. For \eg gradient descent moves into a small sub-space after a few iterations \cite{gur2018gradient}, critical periods where data poising can lead to irreparable generalization error \cite{achille2018critical},  the eigen values of the Hessian grow rapidly and oscillate in the early phase before decaying slowly \cite{jastrzebski2018on}.
%
% (I want to add a more general line here, along the lines of that one would believe they can get away with more approximate gradient apart from these critical regimes) 
%
% \paragraph*{Our contributions}
% \begin{itemize}
%     \item Building on the existence of critical regimes we show that instead of using low compression ratio throughout one just need to use low compression  ratios in these critical regimes
%     \item We empirically show that these critical periods can be easily identified with rapid decrease in gradient norm
%     \item We propose AdaSparse which automatically identifies these critical regimes uses low compression in these regimes and high compression elsewhere.
%     \item AdaSparse when tested on state of the art gradient compression schemes reduces communication by upto 3.7x and training time by 3.6x while keeping the same model accuracy.
% \end{itemize}
% We show our approach can achieve similar accuracy as of using low sparsification during whole of neural network training.
% But further reduce communication upto 3.7x and total training time upto 3.6x when compared to using low sparsification all along. 
% %
% Apart from reducing the total communication our method can significantly reduce the amount of hyper-parameter tuning required as one can easily estimate two values, a lower sparsification factor which leads to no accuracy loss and a high sparsification factor which leads to some accuracy loss.
%Question:(Should we put the our contributions as bullet points)
%There are two points still missing in the introduction 
% one is that it requires considerable amount of tuning to find the right sparsification factors i have tried to put in the end but it would be nicer to put this in problem statement
% second point is about the fact that ten epoch communication is known so helps 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\textwidth]{Figures/critical_regime_effect.pdf}
%     \caption{{\color{red}[DP: add backslash-small to all captions]}Effect of Critical Regimes on Training for ResNet-18, Cifar-10\kw{CIFAR}: (left) We show that critical regimes can be identified with rapid drop in gradients\kw{norms or magnitudes}. \kw{Need to mention that you are assuming powerSGD here} (right) Shows the effect of keeping\kw{choosing? employing?} different compression ratios based on critical regimes. We show that keeping a higher rank (better estimate of the gradient) in the critical regimes and lower rank elsewhere is sufficient to reach the same accuracy as keeping high rank throughout. Further keeping low rank in these regimes is detrimental to the accuracy and can not be compensated with high rank elsewhere \kw{To further highlight the importance of maintaining a low compression rate in these critical regimes, we also test a scheme where a high compression rate is chosen only within those critical regimes, while a low compression rate is used elsewhere. Even though the average compression rate is very low, one can observe that ...} \kw{Also, I think it will be great if we can add `time-average' compression ratio here in the figure.}}
%     \label{fig:critical_regimes}
% \end{figure}



==> introduction.tex <==
\section{Introduction}

Billion-parameter scale neural networks and the rapid increase in compute requirements for training them, has made distributed gradient-based methods a necessity. 
%
Synchronous, data-parallel training is the most widely adopted approach in this context, and requires combining per-node gradient updates every iteration~\cite{dean2012comm, iandola2016firecaffe, goyal2017accurate, shallue2018measuring}.
%(QUESTION: do we need to go a bit more detail about communication, like how much and how often)
Frequently communicating gradients of millions of parameters, across large number of nodes leads to sub-optimal scalability in distributed implementations~\cite{dean2012comm, seide20141bit, alistarh2017qsgd, dawn2019scale, luo2020plink}.
%
% overheads that cause

To alleviate gradient communication bottlenecks, the community has largely focused on two areas, enabling large batch training and lossy gradient compression.
In large batch training each node computes gradients on a larger than usual mini-batch before syncing the gradients among different nodes. Large-batch training can significantly reduces communication frequency. 
It is a widely observed phenomenon that using large batch size leads to degradation in final accuracy~\cite{keskar2016large, yao2018hess, goyal2017accurate, golmant2018computational, shallue2018measuring}. Various previous works have proposed techniques to mitigate this accuracy loss. \cite{goyal2017accurate} use Learning Rate (LR) warmup, while ~\cite{yao2018large, yao2018hess} use second order information. ~\cite{smith2017don, devarakonda2017adabatch} propose hybrid increasing of batch size and LR. Recently~\cite{you2017scaling} use layer wise LR tuning to enable large batches. These methods either end up requiring more epochs to converge to a good accuracy or require significant amount of hyper-parameter tuning, an aspect which is often not discussed~\cite{golmant2018computational, shallue2018measuring}. In our experiments we observe that using a batch size of 4096 compared to using batch size of 512 with LR warmup as proposed by ~\cite{goyal2017accurate} leads to accuracy loss of 1.3\% on \cifart. 
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/accuracy_critical_regions_resnet18_cifar100.pdf}
    \caption{\small{\textbf{Effect of gradient compression in Critical Regimes when Training ResNet-18 on \cifarh:} We conduct these on a 4 Node cluster using \powersgd\ \textsc{Rank 2} (low compression) and \textsc{Rank 1} (high compression) (left) Accuracy vs Epochs, there exist a compression pattern which provides similar training accuracy as using low compression(\textsc{Rank 2}) throughout. (right) Accuracy vs Floats Communicated, this compression pattern communicates significantly less than using low compression throughout (\textsc{Rank 2}) }}
    \label{fig:critical_regimes_cifar100}
    \vspace{-0.1in}
\end{figure*}

For  gradient compression one of the most popular technique is low-precision training which has been heavily studied in past few years \cite{alistarh2017qsgd, seide20141bit, wen2017terngrad, bernstein2018signsgd, acharya2019distributed}.
%
Another line of work~\cite{aji2017sparse, shi2019distributed, shi2019understanding, lin2017deep} exchanges only the largest gradient coordinates. 
These methods are usually referred to as \topk\ where \textsc{K} refers to the total number of coordinates communicated per iteration. 
%
Recently, \cite{wang2018atomo, vogels2019powersgd} have shown how to perform efficient gradient compression using extremely low-rank updates.
% \powersgd\cite{vogels2019powersgd} is a practical low rank method providing end to end speedup.
 %
To alleviate the problem of bias in compressed gradients \citep{stich2018sparsified, stich2019error} utilize error feedback that leads to improved convergence.
%Other work to reduce communication focus on reducing the frequency of gradient updates \cite{stich2019local, wang2020overlap}.
%Not sure if we need the local sgd stuff

% require choosing
All the proposed methods for gradient compression use an extra hyper-parameter which determines the compression or sparsification ratio before training begins.
%
For instance, \topk~\cite{aji2017sparse} requires choosing a hyperparamter \textsc{K} that denotes the number of large-magnitude entries that are going to be communicated in each iteration.  
%
Similarly \powersgd~\cite{vogels2019powersgd}, a low-rank approximation method, requires choosing the rank for the low rank approximation.
%
Choosing compression ratios presents a seemingly inherent trade-off between final model accuracy and per iteration communication overhead. 
%\kw{By carefully choosing compression ratios for these algortihms, one can strike a balance between the final model accuracy and the per-iteration communication overhead.}
%
For instance, training ResNet-18 on \cifart\ using \topk 10\% sparsification takes around 3.6$\times$ less wall-clock time than training using \topk 99\%, but causes around 1.5\% degradation in final accuracy.  Similar trade-offs are observed in~\cite{vogels2019powersgd, alistarh2017qsgd, wang2018atomo, aji2017sparse}.
%

This raises a fundamental question:  \textit{Is this observed trade-off between communication and accuracy fundamental?}  
In this work, we first show that such a trade-off is \emph{not} fundamental but a mere artifact of using a fixed communication scheme throughout training.
In other words, if a gradient compression rate is chosen carefully, like it is done for learning rate or batch size~\cite{smith2017cyclical,Liu2020On, duchi2011adaptive, loshchilov2016sgdr, kingma2014adam, goyal2017accurate}, then  both the final model performance and communication efficiency can be improved, when compared against fixed gradient compression rate throughout training.
Figure~\ref{fig:critical_regimes_cifar100} shows an experiment where we train ResNet-18 on \cifarh, with different compression schemes.  We see that there exists an adaptive compression scheme that significantly reduces communication while maintaining final test accuracy.  Further we show in \Cref{fig:critical_batchsize} that this same scheme allows us to train ResNet-18 on \cifart\ with extremely large batch sizes without loosing accuracy or requiring hyper-parameter tuning.



% In other words, if one can carefully choose a gradient compression rate schedule, as we do for learning rate or batchsize~\cite{smith2017cyclical,Liu2020On, duchi2011adaptive, loshchilov2016sgdr, kingma2014adam, goyal2017accurate}, then one can indeed improve both the final model performance and communication efficiency, compared to the cases where a fixed gradient compression rate is used throughout training.


Our finding -- that there exists a communication-effective adaptive gradient communication scheme that does not hurt the final test accuracy -- is closely related to recent findings made in the deep learning literature. 
In recent work by~\citet{achille2018critical}, the authors show the existence of so-called \emph{critical regimes}, an early phase of training where adding small noise to the data can affect the regions to which training algorithms are steered to in later phases of training, often resulting in poor generalization.
% This is coherent with our finding that there exist certain critical regimes where using a high gradient compression ratio or large batch size can significantly affect the final test accuracy.  % as our algorithm is also based on the observation
% % in which gradient compression does hurt the final generalization performance as well as \emph{non-critical regimes} in which compression does not affect much.
% % We remark that our finding is consistent with recent findings made in the literature.
% \shivaram{remove this part? because we already talked about batch size?}
% Furthermore, our finding is also consistent with the recent findings about the effect of batch-size scheduling on the final test accuracy. 
% In~\cite{goyal2017accurate, devarakonda2017adabatch, you2017scaling, smith2017don}, the authors have shown that the final test accuracy is significantly impaired if large mini-batches are used in early phase of training.
% Moreover, they show that the final test accuracy is not affected even when large batch size is used in later phase of training.
% This is also closely related to our finding and we show that there exists an implicit equivalence between gradient compression and large-batch training under certain conditions.


% how one can 
While our finding implies the existence of adaptive communication schedules, there remain challenges in designing an adaptive compression strategy that is generic across models and compression schemes while imposing low computational overheads. 
We propose \adasp, a simple but powerful gradient communication scheduling algorithm, which can be applied to any existing distributed SGD setup for tuning gradient compression or batch size. 
\adasp\ first identifies whether the current training regime is critical or non-critical by inspecting the change in the gradient norms, and then accordingly adjusts the gradient compression rate.
% Via extensive experiments, we first show that \adasp\ can reliably identify whether or not training is in critical regimes.
We show that \adasp\ can achieve improved communication efficiency while maintaining high generalization performance on computer vision and language modelling tasks. 
In particular, using the SOTA sparsification (\topk) and low-rank approximation methods (\powersgd), we show reduction in communication upto 3.7$\times$ and speedup upto 3.6$\times$ compared to using low compression throughout, while achieving similar accuracy. Further we also extend \adasp\ to perform automated batch size scheduling, we show that \textit{without any hyper-parameter tuning} \adasp\ is able to utilize extremely large batch size leading to reduction in communication of upto $5.5\times$ and speedup of $4.4\times$.  % as using low compression.

\noindent{\textbf{Contributions:}}
\begin{itemize}
    \item We show that there exist an adaptive gradient communication scheme which can achieve the same accuracy as low compression/small batchsize by adaptively switiching between lower and higher compression scheme.
    \item We present \adasp\ an adaptive gradient communication scheduling scheme which can  significantly reduce communication by either using large batch training or gradient compression.
    \item We provide extensive empirical evaluation of \adasp\ on several different neural networks using \powersgd\ and \topk\, two state of the art gradient compressors with different data sets (\cifart, \cifarh, WikiText-2) showing \adasp\ reduces communication significantly without loss of accuracy or change in hyper-parameters.  
    \item We show \adasp\ can enable large batch training by switching between large batch size and small batch size.  \adasp\ \textit{without any hyper-parameter tuning} is able to maintain same accuracy as using a small batch size.
    Moreover \adasp converges while performing up to 5x fewer updates compared to using a small batch size, thereby reducing the time to accuracy.
    % \item \shivaram{Unclear where this comes from.. Remove this?}In a very limited setting we show that there exist an equivalence between large batch training and gradient compression.
\end{itemize}

\section{Introduction 2}
Billion-parameter scale neural networks and the rapid increase in compute requirements for training them, has made distributed gradient-based methods a necessity. 
%
Synchronous, data-parallel training is the most widely adopted approach in this context, and requires combining per-node gradient updates every iteration~\cite{dean2012comm, iandola2016firecaffe, goyal2017accurate, shallue2018measuring}.
%(QUESTION: do we need to go a bit more detail about communication, like how much and how often)
Frequently communicating gradients of millions of parameters, across large number of nodes leads to sub-optimal scalability in distributed implementations~\cite{dean2012comm, seide20141bit, alistarh2017qsgd, dawn2019scale, luo2020plink}.

% To alleviate gradient communication bottleneck, there are primarily two techniques- Gradient Compression and Large batch size training.  In Large batch training each participating worker node computes gradient for a much larger mini-batch size before computing. If large batch training is performed for the same number of epochs as small batch training, then training can be completed in much fewer communication rounds. On the other hand gradient compression methods reduce communication by performing  lossy compression on the gradients thereby reducing the size of the gradient communicated. 

To alleviate gradient communication bottleneck, there are primarily two techniques- Large Batch training and  Lossy Gradient Compression, \ie sparsification, quantization and low-rank updates.  In Large Batch Training each participating worker node computes gradient for a much larger mini-batch size before communicating gradients. If large batch training is performed for the same number of epochs as small batch training, then training can be completed in fewer communication rounds. On the other hand gradient compression methods reduce communication by performing lossy compression of the gradients leading to reduction in the size of the gradient communicated. 

It is a widely observed phenomenon~\cite{goyal2017accurate, vogels2019powersgd, wang2018atomo, alistarh2017qsgd, you2017scaling, keskar2016large, bernstein2018signsgd, seide20141bit, smith2017don, yao2018large} that using extremely large batch training or very high gradient compression can leads to poor test accuracy. In our experiments we observed ResNet-18 on \cifarh\ when trained with Batch size of 4096  with LR warmup~\cite{goyal2017accurate}(a standard technique) for training  observe 3\% accuracy loss compared to training with batch size of 512. Similarly for \powersgd\ (a gradient compression technique) training with Rank-1, Batch size-512 leads to an accuracy loss 2\% when compared to training with Rank-2, Batch size-512 on ResNet-18 and \cifarh. 

There have been various techniques proposed to enable large batch training but either they require significant amount of hyper-parameter tuning~\cite{goyal2017accurate, smith2017don, devarakonda2017adabatch} or require second order information~\cite{yao2018hess, yao2018large}. Similarly gradient compression techniques require choosing a static compression ratio such as Rank for \powersgd~\cite{vogels2019powersgd}, or K\% for \topk~\cite{aji2017sparse} before training. This compression ratio is chosen to provide similar accuracy as syncSGD while reducing gradient communication.

In this work we first show that if gradient communication schedule is chosen carefully, by switching between low communication and high communication then neural network training, without any hyper-parameter tuning can reach the same accuracy as using high communication throughout. Our work is primarily motivated by ~\citet{achille2018critical} and ~\citet{jastrzebski2018on} who show that there exist \textit{critical regimes} in neural network training. And it is in these regimes that majority of the learning happens. We discover that their insight can be extended to gradient communication as well. We show in ~\Cref{fig:critical_regimes_cifar100} that by maintaining high communication(more accurate gradients) only in these \textit{critical regimes} and low communication elsewhere we can achieve the same accuracy as maintaining high communication throughout training. 

While our findings imply the existence of adaptive communication schedules, the challenge still remains in designing adaptive communication strategy that is generic across models and communication schemes. In previous work ~\citet{jastrzebski2018on} used eigen values of the Hessian to identify critical regimes, which requires calculation of second order statistics making it extremely computationally expensive. As shown in ~\Cref{fig:critical_compare}, we observe that rate of change of gradient norm can be used to approximately infer critical regimes.  This enables us to propose \adasp\ a simple yet powerful gradient communication scheduling algorithm. \adasp\ tracks the rate of change of gradient norm to infer critical regimes and switch between low and high communication accordingly. We show that allowing \adasp\ to adaptively switch between low and high communication can provide upto $5\times$ reduction in communication and upto $4\times$ reduction in wall clock timing.

\noindent{\textbf{Contributions:}}
\begin{itemize}
    \item We show that there exist an adaptive gradient communication scheme which can achieve the same accuracy as low compression/small batchsize by adaptively switiching between lower and higher compression scheme.
    \item We present \adasp\ an adaptive gradient communication scheduling scheme which can  significantly reduce communication by either using large batch training or gradient compression.
    \item We provide extensive empirical evaluation of \adasp\ on several different neural networks using \powersgd\ and \topk\, two state of the art gradient compressors with different data sets (\cifart, \cifarh, WikiText-2) showing \adasp\ reduces communication significantly without loss of accuracy or change in hyper-parameters.  
    \item We show \adasp\ can enable large batch training by switching between large batch size and small batch size.  \adasp\ \textit{without any hyper-parameter tuning} is able to maintain same accuracy as using a small batch size.
    Moreover \adasp converges while performing up to 5x fewer updates compared to using a small batch size, thereby reducing the time to accuracy.
\end{itemize}

% Billion-parameter scale neural networks and the rapid increase in compute requirements for training them, has made distributed gradient-based methods a necessity. 
% %
% Synchronous, data-parallel training is the most widely adopted approach in this context, and requires combining per-node gradient updates every iteration~\cite{dean2012comm, iandola2016firecaffe, goyal2017accurate, shallue2018measuring}.
% %(QUESTION: do we need to go a bit more detail about communication, like how much and how often)
% Frequently communicating gradients of millions of parameters, across large number of nodes leads to sub-optimal scalability in distributed implementations~\cite{dean2012comm, seide20141bit, alistarh2017qsgd, dawn2019scale, luo2020plink}.To alleviate these gradient communication bottlenecks, there are primarily two techniques- large batch training and lossy gradient compression. 

% It is a widely observed phenomenon that using large batch size leads to degradation in final accuracy~\cite{keskar2016large, yao2018hess, goyal2017accurate, golmant2018computational, shallue2018measuring}. Various previous works have proposed techniques to mitigate this accuracy loss- Learning Rate (LR) warmup~\cite{goyal2017accurate}, second order information~\cite{yao2018large, yao2018hess}, Hybrid increasing of batch size and LR ~\cite{smith2017don, devarakonda2017adabatch} and layer wise LR tuning~\cite{you2017scaling}. These methods either work only on specific datasets or require significant amount of hyper-parameter tuning an aspect often not discussed~\cite{golmant2018computational, shallue2018measuring}.

% On the other hand everal methods for gradient compression have been proposed. One of the most popular ways to achieve gradient compression is low-precision training that has been heavily studied in past few years \cite{alistarh2017qsgd, seide20141bit, wen2017terngrad, bernstein2018signsgd, acharya2019distributed}.
% %
% Another line of work~\cite{aji2017sparse, shi2019distributed, shi2019understanding, lin2017deep} exchanges only the largest gradient coordinates. 
% These methods are usually referred to as \topk\ where \textsc{K} refers to the total number of coordinates communicated per iteration. 
% %
% Recently, \cite{wang2018atomo, vogels2019powersgd} have shown how to perform efficient gradient compression using extremely low-rank updates.
% % \powersgd\cite{vogels2019powersgd} is a practical low rank method providing end to end speedup.
%  %
% To alleviate the problem of bias in compressed gradients \citep{stich2018sparsified, stich2019error} utilize error feed-back that fixes biases and leads to improved convergence.


% All the proposed gradient compression methods  use an extra hyper-parameter which determines the compression or sparsification ratio before training begins.
% %
% For instance, \topk~\cite{aji2017sparse} requires choosing a hyperparamter \textsc{K} that denotes the number of large-magnitude entries that are going to be communicated in each iteration.  
% %
% Similarly \powersgd~\cite{vogels2019powersgd}, a low-rank approximation method, requires choosing the rank for the low rank approximation.
% %
% Choosing compression ratios presents a seemingly inherent trade-off between final model accuracy and per iteration communication overhead. 
% %\kw{By carefully choosing compression ratios for these algortihms, one can strike a balance between the final model accuracy and the per-iteration communication overhead.}
% %
% For instance, training ResNet-18 on \cifart\ using \topk 10\% sparsification takes around 3.6$\times$ less wall-clock time than training using \topk 99\%, but causes around 1.5\% degradation in final accuracy.  Similar trade-offs are observed in~\cite{vogels2019powersgd, alistarh2017qsgd, wang2018atomo, aji2017sparse}.
% %

% This raises a fundamental question:  \textit{Is this observed trade-off fundamental?}  
% In this work, we first show that such a trade-off is \emph{not} fundamental but a mere artifact of using a fixed compression rate throughout training.
% In other words, if a gradient compression rate is chosen carefully, like it is done for learning rate or batch size~\cite{smith2017cyclical,Liu2020On, duchi2011adaptive, loshchilov2016sgdr, kingma2014adam, goyal2017accurate, smith2017don}, then  both the final model performance and communication efficiency can be improved, when compared against fixed gradient compression rate throughout training.
% Figure~\ref{fig:critical_regimes_cifar100} shows an experiment where we train ResNet-18 on \cifarh, with different compression schemes.  We see that there exists an adaptive compression scheme that can significantly reduces communication while maintaining final test accuracy. 



% % In other words, if one can carefully choose a gradient compression rate schedule, as we do for learning rate or batchsize~\cite{smith2017cyclical,Liu2020On, duchi2011adaptive, loshchilov2016sgdr, kingma2014adam, goyal2017accurate}, then one can indeed improve both the final model performance and communication efficiency, compared to the cases where a fixed gradient compression rate is used throughout training.


% Our finding -- that there exists a communication-effective adaptive gradient compression scheme that does not hurt the final test accuracy -- is closely related to recent findings made in the deep learning literature. 
% In recent work by~\citet{achille2018critical}, the authors show the existence of so-called \emph{critical regimes}, an early phase of training where adding small noise to the data can affect the regions to which training algorithms are steered to in later phases of training, often resulting in poor generalization.
% This is coherent with our finding that there exist certain critical regimes where using a high gradient compression ratio can significantly affect the final test accuracy.  % as our algorithm is also based on the observation
% % in which gradient compression does hurt the final generalization performance as well as \emph{non-critical regimes} in which compression does not affect much.
% % We remark that our finding is consistent with recent findings made in the literature.
% Furthermore, our finding is also consistent with recent findings about the effect of batch-size scheduling on the final test accuracy. 
% In~\cite{goyal2017accurate, devarakonda2017adabatch}, the authors have shown that the final test accuracy is significantly impaired if large mini-batches are used in early phase of training.
% Moreover, they show that the final test accuracy is not affected even when large batch size is used in later phase of training. 
% This is also closely related to our finding and we show that there exists an implicit equivalence between gradient compression and large-batch training under certain conditions.  


% % how one can 
% While our finding implies the existence of effective adaptive compression schedules, there remain challenges in designing an adaptive compression strategy that is generic across models and compression schemes while imposing low computational overheads. 
% We propose \adasp, a simple but powerful gradient compression scheduling algorithm, which can be applied to any existing distributed SGD setup with any gradient compression scheme. 
% \adasp\ first identifies whether the current training regime is critical or non-critical by inspecting the change in the gradient norms, and then accordingly adjusts the gradient compression rate.
% % Via extensive experiments, we first show that \adasp\ can reliably identify whether or not training is in critical regimes.
% We show that \adasp\ can achieve improved communication efficiency while maintaining high generalization performance on computer vision and language modelling tasks. 
% In particular, using the SOTA sparsification (\topk) and low-rank approximation methods (\powersgd), we show reduction in communication upto 3.7$\times$ and speedup upto 3.6$\times$ compared to using low compression throughout, while achieving similar accuracy. % as using low compression.


% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.9\textwidth]{Figures/accuracy_critical_regions_resnet18_cifar100.pdf}
%     \caption{\small{\textbf{Effect of gradient compression in Critical Regimes when Training ResNet-18 on \cifarh:} We conduct these on a 4 Node cluster using \powersgd\ \textsc{Rank 2} (low compression) and \textsc{Rank 1} (high compression) (left) Accuracy vs Epochs, there exist a compression pattern which provides similar training accuracy as using low compression(\textsc{Rank 2}) throughout. (right) Accuracy vs Floats Communicated, this compression pattern communicates significantly less than using low compression throughout (\textsc{Rank 2}) }}
%     \label{fig:critical_regimes_cifar100}
%     \vspace{-0.1in}
% \end{figure*}




% \begin{figure}[t]
%     \begin{center}
%     \begin{subfigure}[b]{0.49\textwidth}
%         \includegraphics[width=0.9\textwidth]{Figures/accuracy_critical_regions_resnet18.pdf}
%         \caption{Effect of using different Compression Ratios in Critical Regimes on (left)accuracy vs Epochs and (right)Accuracy vs Floats communication }
%         \vspace{-0.1in}
%         \label{fig:1a}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.49\textwidth}
%         \includegraphics[width=0.9\textwidth]{Figures/accuracy_critical_regions_resnet18_cifar100.pdf}
%         \caption{Critical Regions}
%         \vspace{-0.03in}
%         \label{fig:1b}
%     \end{subfigure}
%     % \begin{subfigure}[b]{0.9\textwidth}
%     %     \includegraphics[width=0.9\textwidth]{Figures/psgd_senet_cifar10.pdf}
%     %     \caption{Cifar10, SeNet}
%     % \end{subfigure}
%     \end{center}
%     \caption{\small{\textbf{Effect of Gradient Compression in Critical Regimes when Training ResNet-18 on \cifart:} This experiment was performed for 4 Nodes (a) We show that critical regimes can be identified with rapid change in gradient norm. (b, left) Shows the effect of running \powersgd\ with different compression ratios and it's  effect on final accuracy. It can be observed that keeping \mbox{\textsc{Rank 4}} (better estimate of the gradient, lower Compression) in the critical regimes and \mbox{\textsc{Rank 1}} (poor estimate of the gradient, Higher Compression) elsewhere is sufficient to reach the same accuracy as keeping \mbox{\textsc{Rank 4}} throughout. Further keeping \mbox{\textsc{Rank 1}} in these critical regimes is detrimental to the accuracy and can not be compensated with \textsc{Rank 4} elsewhere. %To further highlight the importance of maintaining a low compression rate in these critical regimes, we also test a scheme where \mbox{\textsc{Rank 1}} is chosen only within those critical regimes, while \mbox{\textsc{Rank 4}} is used elsewhere. 
%     (b,right) Shows Accuracy vs Float communicated, even though the communication is high for using \textsc{Rank 1} in critical regimes and \textsc{Rank 4} otherwise, there is significant drop in Test Accuracy. This shows the relationship between Communication and Accuracy is not linear. \ie more Communication doesn't imply better Test Performance}}
%     \label{fig:critical_regimes}
%     \vspace{-0.26in}
% \end{figure}


%
% We employ these insights to gradient compression:
% as long as we're outside of a critical learning regime, low accuracy gradients are sufficient for training, but should be avoided once in it. We validate these insights in Figure~\ref{fig:critical_regimes}, where we show that if we over-compress gradients during these critical regimes, then test accuracy is significantly impaired.
% %
% On the other hand, we show that when compression ratios are selected conservatively to avoid impairing the training process during these critical regimes, then test error is unaffected, even if high compression is used in other regimes.
% %
% %Furthermore, we propose a simple method that identifies such critical regimes by continuously inspecting the scale of gradient norms while training . 
% {\color{red}[DP: I want to add that folks may complain here and say, how does fast gradient change relate to the literature. Can you ellaborate on this] \address{I am not aware of literature around fast gradient change i tried to look couldn't find something}}
% %

% Inspired by these observations, we propose \adasp\ an online algorithm that automatically identifies critical regimes and accordingly switches between low/high compression modes.
% %
% Unlike the computationally expensive methods of~\cite{keskar2016large, Jastrzebski2020The} where critical regimes are characterized by eigenvalues of the Hessian matrix, \adasp\ uses rate of change in gradient norm to identify critical regime.
% %
% This makes \adasp's computational overhead almost negligible.
% %TODO: Formulate the 
% %
% We evaluate training performance of \adasp\ on computer vision and language modelling tasks. 
% %

%Keeping the sparsification constant throughout training is at odds with recent work which has shown presence of critical regimes in neural network training, since one would assume that these regimes 
%
% It has been suggested that various important aspects of training occur in early phase of neural network training. For \eg gradient descent moves into a small sub-space after a few iterations \cite{gur2018gradient}, critical periods where data poising can lead to irreparable generalization error \cite{achille2018critical},  the eigen values of the Hessian grow rapidly and oscillate in the early phase before decaying slowly \cite{jastrzebski2018on}.
%
% (I want to add a more general line here, along the lines of that one would believe they can get away with more approximate gradient apart from these critical regimes) 
%
% \paragraph*{Our contributions}
% \begin{itemize}
%     \item Building on the existence of critical regimes we show that instead of using low compression ratio throughout one just need to use low compression  ratios in these critical regimes
%     \item We empirically show that these critical periods can be easily identified with rapid decrease in gradient norm
%     \item We propose AdaSparse which automatically identifies these critical regimes uses low compression in these regimes and high compression elsewhere.
%     \item AdaSparse when tested on state of the art gradient compression schemes reduces communication by upto 3.7x and training time by 3.6x while keeping the same model accuracy.
% \end{itemize}
% We show our approach can achieve similar accuracy as of using low sparsification during whole of neural network training.
% But further reduce communication upto 3.7x and total training time upto 3.6x when compared to using low sparsification all along. 
% %
% Apart from reducing the total communication our method can significantly reduce the amount of hyper-parameter tuning required as one can easily estimate two values, a lower sparsification factor which leads to no accuracy loss and a high sparsification factor which leads to some accuracy loss.
%Question:(Should we put the our contributions as bullet points)
%There are two points still missing in the introduction 
% one is that it requires considerable amount of tuning to find the right sparsification factors i have tried to put in the end but it would be nicer to put this in problem statement
% second point is about the fact that ten epoch communication is known so helps 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\textwidth]{Figures/critical_regime_effect.pdf}
%     \caption{{\color{red}[DP: add backslash-small to all captions]}Effect of Critical Regimes on Training for ResNet-18, Cifar-10\kw{CIFAR}: (left) We show that critical regimes can be identified with rapid drop in gradients\kw{norms or magnitudes}. \kw{Need to mention that you are assuming powerSGD here} (right) Shows the effect of keeping\kw{choosing? employing?} different compression ratios based on critical regimes. We show that keeping a higher rank (better estimate of the gradient) in the critical regimes and lower rank elsewhere is sufficient to reach the same accuracy as keeping high rank throughout. Further keeping low rank in these regimes is detrimental to the accuracy and can not be compensated with high rank elsewhere \kw{To further highlight the importance of maintaining a low compression rate in these critical regimes, we also test a scheme where a high compression rate is chosen only within those critical regimes, while a low compression rate is used elsewhere. Even though the average compression rate is very low, one can observe that ...} \kw{Also, I think it will be great if we can add `time-average' compression ratio here in the figure.}}
%     \label{fig:critical_regimes}
% \end{figure}


